WiForceSticker: Batteryless, Thin Sticker-like Flexible Force Sensor

Any two objects in contact with each other exert a force that could be simply due to gravity or mechanical contact, such as a robotic arm gripping an object or even the contact between two bones at our knee joints. The ability to naturally measure and monitor these contact forces allows a plethora of applications from warehouse management (detect faulty packages based on weights) to robotics (making a robotic arms' grip as sensitive as human skin) and healthcare (knee-implants). It is challenging to design a ubiquitous force sensor that can be used naturally for all these applications. First, the sensor should be small enough to fit in narrow spaces. Next, we don't want to lay cumbersome cables to read the force values from the sensors. Finally, we need to have a battery-free design to meet the in-vivo applications. We develop WiForceSticker, a wireless, battery-free, sticker-like force sensor that can be ubiquitously deployed on any surface, such as all warehouse packages, robotic arms, and knee joints. WiForceSticker first designs a tiny $4$~mm~$\times$~$2$~mm~$\times$~$0.4$~mm capacitative sensor design equipped with a $10$~mm~$\times$~$10$~mm antenna designed on a flexible PCB substrate. Secondly, it introduces a new mechanism to transduce the force information on ambient RF radiations that can be read by a remotely located reader wirelessly without requiring any battery or active components at the force sensor, by interfacing the sensors with COTS RFID systems. The sensor can detect forces in the range of $0$-$6$~N with sensing accuracy of $<0.5$~N across multiple testing environments and evaluated with over $10,000$ varying force level presses on the sensor. We also showcase two application case studies with our designed sensors, weighing warehouse packages and sensing forces applied by bone joints.

==> background/background.tex <==
% !TEX root = paper.tex

% intro needs to motivate mm scale force sensors

\section{Background and Motivation}\label{sec:background}

% resistive sensors cant be miniaturized
% we need capacitative sensors
% naive way of reading such sensors: use a CDC
% we show how we can do wireless

% Cant be miniaturized <1GHz

% sensor designs: quantity trasnduces to change in impedance/resistive/capacitative etc etc
% backscatter sensing modalities: expose digital outputs. attempts at integrating these require 

% A common theme in building today's force sensors has been to create transduction mechanisms which lead to changes in impedance, which can then be measured 
\subsection{Sensors which solve for space constraints}
Today's force sensors typically use either resistive \cite{} or capacitative transduction mechanisms \cite{}. 
The basic principle of operation is that as force is applied on these sensors, they respond with changes in impedance, which can be then measured and digitized electrically.
In order to sense the resistive transduction
we need to power up the resistive sensor via a DC power supply VCC for sensing purposes, as the change in resistance (and hence the change in force) is sensed by observing the change in the DC current/voltage consumed by the sensor.
These changes in DC current/voltage levels can be readily captured by ADCs to digitize the sensor information.

Capacitative sensors on the other hand do not require a DC power supply, and are typically read by exciting the capacitor with a low frequency ($\sim$ kHz) voltage and then measuring the stored charges in the capacitor as a response to the excitation. The device which enables this excitation and charge storage mechanism is also referred to as a CDC (Capacitance to Digital Converter)~\cite{}.

In addition to being low-powered, capacitative sensors also offer better miniaturized sensors. When the resistive sensors scale down in size, the resistance typically decreases, and this leads to both, a higher power consumption in the sensor itself due to reduced resistance, and reduced sensitivity as the net change in resistance reduces as well~\cite{}.
In comparison, capacitative sensors offer better charge retention with miniaturization, as this leads to an increase in capacitance (due to capacitor electrodes being closer to each other) and thus do not suffer from increased power consumption and reduced sensitivity due to miniaturization as compared to resistive sensors~\cite{}.

\subsection{Sensors which solve for energy constraints}
The naive way of interfacing these resistive/capacitative force sensors to wireless sensing modalities is to take the digital data from the ADC/CDC and communicate them via wireless communication technologies.
BLE has typically been used to achieve the same ~\cite{}, however it requires a battery which prohibits the sensor miniaturization as well as practical usages of the sensor.
Low power wireless technologies which are battery-free like NFC, RFID and backscatter offer an interesting alternative to the commonly deployed BLE.

There are some force sensors integrated with NFC wireless technology ~\cite{}, however NFC has very low range in order of few centimeters.
UHF RFID in 900 MHz range and WiFi based backscatter can be used to feedback the digital sensor data over practically viable distances but there are no practical demonstrations for force sensors with these technologies today.
A key reason is that these technologies typically allow sensor interfacing via integrated ADCs which can be used with resistive force sensors, but not with capacitative sensors. 
However, inherently the resistive force sensors require power drain and thus are not low-powered and thus can not be used simply with these backscatter technologies without adding to the power consumption.
Infact, ~\cite{} shows the challenges of integrating such resistive sensors with UHF RFIDs, as adding these sensors has an adverse effect on the read ranges among other practical problems.

Hence, the gold standard is to somehow integrate the capacitative sensor with these low-power wireless backscattering technologies.
A naive solution is to simply take the CDCs today and then communicate the digital data.
This however requires an redesign of the low-power microcontrollers in these backscattering ICs to include CDCs in addition to ADCs, which has not been demonstrated yet.
In \name we show how capacitative force senor can be integrated much more easily with currently existing RFID tags without requiring any redesign and truly enabling the low-power miniaturized wireless force sensing applications.

% There have been a lot of research in sensor design \cite{} which ultimately cause some impedance changes due to change in sensing quantity. Parallely, backscatter solutions have become more and more mature with them supporting to and fro data transmissions etc.
% However, how do we 




==> background/bandmv2.tex <==
% !TEX root = paper.tex

% intro needs to motivate mm scale force sensors

\section{Background and Motivation}\label{sec:background}

\subsection{Energy and Space constraint force sensing applications}
% Discussion applications again in a bit more detail and multiple applications carefully... 
% One of the reasons is the technological
% limitation with existing force sensors that these sensors require either a battery, or a tethered wired link to
% sense and communicate these force information. As a consequence, we have only achieved the applications
% where we have the resources to put a battery to enable force sensing, for example, weighing scales, underneath
% our trackpads and even on latest airpods for force based haptic control. But, on these simple and ubiquitous
% objects like bottles, milk cans such sensors would be too impractical and expensive to design. Further,
% requirement of batteries is simply unimaginable for the surgical usecases, as it would be too risky and unsafe
% to carry a battery inside body just to get force information. Hence, in order to lift these roadblocks with
% existing force sensors we design wireless batteryless force sensors.

motivate the requirements a bit more carefully

\subsection{Current Force Transduction Mechanism and Limitations}


% resistive sensors cant be miniaturized
% we need capacitative sensors
% naive way of reading such sensors: use a CDC
% we show how we can do wireless

% Cant be miniaturized <1GHz

% sensor designs: quantity trasnduces to change in impedance/resistive/capacitative etc etc
% backscatter sensing modalities: expose digital outputs. attempts at integrating these require 

% A common theme in building today's force sensors has been to create transduction mechanisms which lead to changes in impedance, which can then be measured 
% \subsection{ in force sensors}

Force sensors has been an active area of research over the past years in the flexible electronics and MEMS sensor communities \cite{}.
Today's force sensors popularly use either resistive \cite{} or capacitative transduction mechanisms \cite{}.  
The basic principle of operation is that as force is applied on these sensors, they respond with changes in impedance, which can be then measured and digitized electrically.

In order to sense the resistive transduction
the typical method is to
% need to power up the resistive sensor via a DC power supply VCC for sensing purposes, as the change in resistance (and hence the change in force) is sensed by observing 
observe the change in the DC current/voltage due to change in resistance, and hence force.
These changes in DC current/voltage levels can be readily captured by ADCs to digitize the sensor information.
On the first look, resistive force sensors offer a good candidate to low-power integration with today's wireless backscatter communication systems, with some advanced platforms exposing ADC pins on an embedded microcontroller ~\cite{}.
Hence one can plug these resistive sensors to the ADCs of today's backscatter systems to get force readings in a batteryless wireless manner.
So hypothetically, resistive sensors + digital backscatter is a viable low-energy force sensor but resistive sensors are incredibly hard to miniaturize and thus these hypothetical prototypes would end up violating the space constraints.
When the resistive sensors scale down in size, the resistance typically decreases, and this leads to both, a higher power consumption in the sensor as more current now flows through the sensor, and reduced sensitivity as the net change in resistance reduces ~\cite{}.

In comparison, capacitative sensors work better as they are miniaturized, since the capacitance increases due to miniaturization as capacitor conductors come closer to each other and the charge retention increases. Hence, these sensors do not suffer from the reduced sensitivity due to miniaturization as compared to resistive sensors~\cite{}.
However, the reading methods for Capacitative sensors are more involved and we can't simply hook up a capacitative sensor to ADC and make it work. Today, the capacitative sensors are typically read by exciting the capacitor with a low frequency ($\sim$ kHz) voltage and then measuring the stored charges in the capacitor as a response to the excitation. The system block which enables this excitation and computation of charge storage mechanism is also referred to as a CDC (Capacitance to Digital Converter)~\cite{}.

Implementing the CDC block in a low-power method compliant with energy requirements of backscatter systems has not been attempted and might require a ground-up redesign of existing backscatter systems. Hence attempts at making capacitative sensors wireless end up using technologies like BLE ~\cite{}, which require battery and end up violating energy constraints.
Hence even though capacitative sensors by themselves allow sensor miniaturization and solve the space constraints, they can not be read easily via ADCs and thus are difficult to integrate with today's backscatter systems, and this ends up violating the energy constraints.

Hence because of this energy-space tradeoff with existing force sensors, resistive sensors have been popularly used where there are no space constraints, for example underneath laptop trackpads for touch gestures \cite{}. The capacitative sensors have been used for space constraint scenarios, like in airpods \cite{} for haptic earbud control, though they use the airpods battery to bypass the energy constraints.
However, owing to difficulties in backscatter integration of these capacitative sensors the medical and robotic applications requiring to solve both these constraints simultaneously remain unfulfilled. 
Thus, the gold standard is to somehow integrate the capacitative sensor with these low-power wireless backscattering technologies.
In \name we show how capacitative force sensors can be integrated much more easily with currently existing RFID tags without requiring any redesign and truly enabling the low-power miniaturized wireless force sensing applications.

% In addition to being low-powered, capacitative sensors also offer better miniaturized sensors. 

\subsection{Meeting Energy and Space}

Leverage RFID and ...

% \subsection{Sensors which solve for energy constraints}
% The naive way of interfacing these resistive/capacitative force sensors to wireless sensing modalities is to take the digital data from the ADC/CDC and communicate them via wireless communication technologies.
% BLE has typically been used to achieve the same ~\cite{}, however it requires a battery which prohibits the sensor miniaturization as well as practical usages of the sensor.
% Low power wireless technologies which are battery-free like NFC, RFID and backscatter offer an interesting alternative to the commonly deployed BLE.

% There are some force sensors integrated with NFC wireless technology ~\cite{}, however NFC has very low range in order of few centimeters.
% UHF RFID in 900 MHz range and WiFi based backscatter can be used to feedback the digital sensor data over practically viable distances but there are no practical demonstrations for force sensors with these technologies today.
% A key reason is that these technologies typically allow sensor interfacing via integrated ADCs which can be used with resistive force sensors, but not with capacitative sensors. 
% However, inherently the resistive force sensors require power drain and thus are not low-powered and thus can not be used simply with these backscatter technologies without adding to the power consumption.
% Infact, ~\cite{} shows the challenges of integrating such resistive sensors with UHF RFIDs, as adding these sensors has an adverse effect on the read ranges among other practical problems.

% Hence, the gold standard is to somehow integrate the capacitative sensor with these low-power wireless backscattering technologies.
% A naive solution is to simply take the CDCs today and then communicate the digital data.
% This however requires an redesign of the low-power microcontrollers in these backscattering ICs to include CDCs in addition to ADCs, which has not been demonstrated yet.
% In \name we show how capacitative force senor can be integrated much more easily with currently existing RFID tags without requiring any redesign and truly enabling the low-power miniaturized wireless force sensing applications.

% There have been a lot of research in sensor design \cite{} which ultimately cause some impedance changes due to change in sensing quantity. Parallely, backscatter solutions have become more and more mature with them supporting to and fro data transmissions etc.
% However, how do we 




==> background/bgm_v3.tex <==
% !TEX root = paper.tex

% intro needs to motivate mm scale force sensors

\section{Background and Motivation}\label{sec:background}

\subsection{Energy and Space constraint force sensing applications require batteryless wireless sensors}
% Discussion applications again in a bit more detail and multiple applications carefully...
% Force sensors has been an active area of research over the past years across various domains like flexible electronics and MEMS sensor communities \cite{}.
A significant technological limitation of existing force sensors is that they require either a battery, or a tethered wired link to
sense and communicate force information. 
As a consequence, applications have been limited to those that have the resources for a battery, including for example weighing scales with load cells\cite{}, force sensitive resistors beneath
our trackpads\cite{} and capacitive force sensors in latest AirPods for haptic based volume control\cite{}. 

There are many applications which demand batteryless force sensors.
For example, studies have shown that incorporation of force feedback in surgical instruments leads to safer surgeries\cite{}.
However, to measure the applied forces, the sensors would need to be batteryless since these surgical equipments would be going inside body and carrying batteries in-vivo has drastic risks\cite{}.
Another similar application involves sensing forces applied to soft and continuum robots, in order to improve their control and operation~\cite{}.
These robots are flexible and have a small form factor since they are often designed for use in surgery \& search and rescue, where they must navigate through highly constrained environments.
Force sensors for these robots must also be small and flexible, and the presence of batteries or wired links make these requirements difficult to meet.

Finally, such sensors could enable new technologies, such as implants equipped with force sensors.
An orthopedic implant equipped with a batteryless force sensor can be monitored in a non-invasive manner. This would allow getting information about the forces applied by the bone joints onto the implant, to ascertain if the implant is handling the forces within the prescribed load limit of the joint.
A common theme to note is that most of the applications for batteryless sensors require sensing in-vivo and from space constrained mounting positions like surgical equipment/robots.
Hence it is required to not only make the sensors batteryless but also miniaturized enough to truly fulfill these applications.
% But, on these simple and ubiquitous
% objects like bottles, milk cans such sensors would be too impractical and expensive to design. Further,
% requirement of batteries is simply unimaginable for the surgical usecases, as it would be too risky and unsafe
% to carry a battery inside body just to get force information. Hence, in order to lift these roadblocks with
% existing force sensors we design wireless batteryless force sensors.

% motivate the requirements a bit more carefully

\subsection{Can existing sensors be miniaturized and made wireless and batteryless?}

Before motivating \name sensor design, we would first motivate why the existing sensors fail to be miniaturized and batteryless simultaneously.
A central idea to making a force sensor wireless and batteryless is to create a joint communication+sensing paradigm.
This essentially requires the sensor to encode the force information onto reflected signals, which create alterations in wireless channel.
A remotely located reader can then estimate the changes in wireless channel to get the force estimates from the sensor.
% Creating these encoding in wireless channel can be created by exploiting how wireless signals at RF frequencies get fundamentally altered due to the forces on the sensor.
As compared to generating and transmitting the signals to communicate the sensor output, conveying the same via reflected signals in this joint communication sensing methodology allows for batteryless wireless operation.

Hence, in order to create batteryless wireless sensors, past works utilize transduction mechanisms which map force to wireless channel properties.
% LC sensors to be handled as well

% The existing gold standard for miniaturized force sensors are the capacitive force sensors~\cite{}.
% Now, to make these sensors batteryless, one approach could be to simply interface this with existing wireless batteryless backscatter systems, which usually have an ADC to interface with external sensors.
% However, the capacitive sensors can not be simply plugged into an ADC to read the capacitances (and hence the force).
% Capacitive force sensors are typically read by exciting the capacitor with a low frequency ($\sim$ kHz) voltage and then measuring the stored charges in the capacitor as a response to the excitation. 
% The device which enables this excitation and charge storage mechanism is also referred to as a CDC (Capacitance to Digital Converter)~\cite{}.
% Now incorporating CDC's with existing backscatter systems would require a ground-up redesign, since none of today's systems have CDC presently.
% Also, integrating this CDC would not be simple, since the power requirements of CDCs are typically in mW whereas backscatter systems need to work with uW power to justify the batteryless operation.
% Hence the best miniaturized sensors today are incompatible with low-power wireless communications.

% Next, we have a set of sensors which utilize direct RF interrogation of force ~\cite{}. Most of these sensors rely on encoding forces onto antenna's resonant frequency \cite{} and using force to contact length mapping to affect the reflected signal phase \cite{}.
% Since both these sensor transduction mechanisms depend on the length phenomenon, either how length change affects antenna's resonance or the signal phase, these batteryless sensors are difficult to miniaturize at sub-1 GHz frequencies which have wavelengths $>$30cm.



% \subsection{Meeting Energy and Space}



==> background/bgm_v4.tex <==
% !TEX root = paper.tex

% intro needs to motivate mm scale force sensors

\section{Background and Motivation}\label{sec:background}

\subsection{Batteryless and sticker-like force sensors allow medical, robotic, and ubiquitous applications}
% \begin{itemize}
%     \item \textbf{Force sensors which can be stuck like stickers on everyday objects; will allow for sensing weight and other applications}
%     \item \textbf{Further such sensors, being batteryless can be used with implants and surgical setting as these can be read wirelessly and thus can lead to scalable deployments}
% \end{itemize}
This battery or tethered power link requirement does not allow scalable deployment of force sensors and limits their possible applications. 
Hence, we can not enable applications that require battery-free wireless sensing, like ubiquitous weight sensing, in-vivo implants, and robots with existing force sensors.

We can use force sensors to measure the weight of contents in a package in warehouse settings to determine empty or incorrectly packed packages.
A naive solution would be to attach these small weighing scales below each package. However this is clearly not scalable, given the form factor, cost and reading of these multiple weighing scales.
On the other hand, a sticker like a battery-free force sensor, which can be read as easily as a barcode, would be a scalable solution as it will solve all the challenges: thin paper-like form factor, negligible cost, and easy automated reading of weight via a scanner like a device.

Due to the thin form factor and batteryless feature, \name is an apt candidate to enable smart force-sensitive implants. 
Today, the field of medical orthopedic implants is already looking to engineering fields for innovation, with personalized 3-d printed implants making a lot of headway.
The implants can be made much smarter by adding these force stickers on top of these 3-d printed structures; since these are highly flexible, the sticker would conform well to the implant's shape and be able to measure the bone joint forces.
There are already research studies motivating the use of force sensors in implants to enable implant health monitoring and sense how well the implant fits within the bone joint~\cite{safaei2018force,s140815009,knee_implant}.
However, these studies were done in laboratory settings with wired force sensors which can not work in-vivo.
\name's batteryless sticker-like force sensors being batteryless would finally enable these in-vivo applications and ubiquitous weight sensing application.

Another application which \name can enable involves sensing forces applied by robots to improve their control and operation~\cite{yip2016model,billard2019trends, deng2020grasping}.
% These robots are flexible and have a small form factor since they are often designed for use in surgery \& search and rescue, where they must navigate through highly constrained environments.
Wired force sensors could hamper the robot's movements and make the robot less flexible.
The problem gets exacerbated with emerging robot designs like soft robots\cite{burgner2015continuum}, which have a highly flexible and small form factor since they are often designed for use in surgery \& search and rescue, where they must navigate through highly constrained environments.
Hence, the ideal force sensors for these robotic applications must also be small and flexible, and the presence of batteries or wired links makes these requirements difficult to meet.
Hence, \name can be stuck to various parts of robot without disturbing the robot motion by much and give the required force feedback for efficient robot control.

\subsection{Can existing sensors be made wireless and stick-like form factor for these applications?}
The existing force sensors are typically MEMS-based discrete sensors that use a variety of transduction mechanisms, like the force-induced change of resistance/capacitance (resistive/capacitive sensors)\cite{capacitivesurvey,capacitivetina,resistive1,resistive2} and piezo current generated due to applied force (piezoelectric sensors)\cite{piezo3,piezo2,piezocatheter}. 
The typical paradigm is to digitize the transduction effect via Analog to Digital Converters (ADCs)\cite{dahiya2011towards,ibrahim2018experimental} or Capacitance to Digital Converters (CDCs)\cite{capacitivetina,kim2015force}, which measure the change in current/resistance and capacitance, respectively.
Now to communicate wirelessly, these digitized values are typically transmitted via digital communication blocks like BLE/Wi-Fi, etc.
This interfacing requires a battery which ends up violating the form factor requirements for sticker-like wireless sensors.
As a consequence, the applications for such force sensors have been limited to those that have the resources for a battery, for example, weighing scales with load cells\cite{weigh_scale}, force-sensitive resistors beneath our trackpads\cite{sensel} and capacitive force sensors in latest AirPods for haptic-based volume control\cite{airpods}. 

Now to make these sensors sticker-like form factor and batteryless, an attractive approach is to interface the sensors to RFIDs.
RFIDs already come in sticker like form-factors and communicate to a RFID reader wihtout any battery by relying on energy harvested via RF signals.
% The most naive approach is to piggyback on the RFID digital communications backbone and communicate the digitized sensor readings in addition to the usual EPC IDs\footnote{a simple identification number to distinguish different RFIDs} communicated by the RFIDs.
% However, it has two issues. First, the typical stickable COTS RFIDs do not have ADC interfaces to directly plug these sensors in~\cite{pradhan2020rtsense}.
% Second, even with some high-end RFIDs having options of sensor integration via on-chip ADCs~\cite{fernandez2015passive,AMSSL900A}, there are extra accompanying electronics to enable sensor data buffering, and data register writing, which put a massive burden on energy harvestor since RFIDs operate on a very tight energy budget.
An approach tried by past work ~\cite{omidRFID} is to directly connect the MEMS sensors to RFID by cutting a small part of the RFID antenna and replacing it with the sensors in series.
Although ~\cite{omidRFID} evaluates this strategy for Temperature/Light sensors, it is still possible in the purview of the suggested RFID hacking to put a small MEMS force sensor using similar cut and interface in series technique.
This is because the chosen MEMS sensors lead to change in sensor impedance due to a change in Temperature/Light, similar to how force sensors change impedance under forces. 
This change in impedance across the cut parts of antenna creates fluctuations in the wake-up thresholds of the energy harvester, and this fluctuation is used as a metric for wireless sensing.
However, this technique hampers the RFID read range in the process as it disturbs the energy harvester, which impacts the quality of the reflected signal and hence the sensor resolution.
In fact, this particular past work ~\cite{omidRFID} poses the sensor integration with RFIDs as a challenge paper, so as to how to integrate the sensors without losing range and resolution in the process.

In this paper, we essentially give a solution to the so-posed challenge by designing a new miniaturized force sensor that works as a purely capacitative sensor. Our key insight is that when we interface this force-sensitive capacitor in parallel to the RFID, it creates pure phase shifts with minimal change in amplitude.
Hence, this does not hamper the amplitude of signal reflections and thus preserves the range of the RFIDs and allows the sensing to go ahead at the highest possible resolution.
Due to this successful RFID integration, we achieve the first force sensors in this sticker-like form factor and demonstrate various applications.

% \begin{itemize}
%     \item \textbf{Existing sensors are typically wired, or battery+wireless and thus not sticker form factor. Presence of wires and battery destroys any chance of sticker form factor}
%     \item \textbf{Closest possible works are, (a) WiForce which was a specialized sensor design requiring careful manufacturing and has air gaps and thus not sticker form factor (b) the LC sensors with inductor coils, which are not robustly read in common environments}
% \end{itemize}

% LC sensors
% WiForce

==> design/design_v1.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}
% \textcolor{blue}{
% So the design can really go 2 ways: we go full blown into doppler suppression for RFID and make it a targeted RFID paper, or we put across the various COTS reader arguments. 
% \begin{itemize}
%   \item The prior approach is more well suited for NSDI 
%   \item The former becomes towards maybe Mobisys demo/Sensys. Also we can include real-life bottle sensing etc applications whereas NSDI can be in general
% \end{itemize}
% Main thing to sell here is the sensor and not the RFID stuff, we will kindof just overlook it and write the paper how Omid et al wrote. 
% So kindof makes sense to demonstrate the prior one for now in next 20 days. List of technologies which can be potentially demonstrated:
% 1. RFID (batteryless robot experiment, knee implant)
% 2. OFDM (show some AR/VR applications use WiForce algo)
% 3. LoRA/nb-IoT
% 4. UWB if possible this will make it slam dunk
% }

\name presents the first miniaturized (mm-scale) capacitative wireless force sensor which seamlessly integrates with any backscatter wireless technology today.
Hence, \name sensor solves for both space and energy constraints with force sensing.
In this section we delinate various facets behind \name.
First, we briefly describe the mm-scale capacitative force sensor used by \name. Then, we show how this sensor can be easily integrated into RF PCBs as a component pad and finally we present the details on how the sensor can feedback force-readings in a batteryless wireless manner by piggybacking on the UHF RFIDs.
% In this section we present the various design facets of \name which enable these features: (1) miniaturized passive , (2) wireless and (3) seamless integrability. 
% First, we explain the sensor design and how it transduces force onto change in impedance. Then, we go into the details on how the sensor can be integrated with RF components, like ICs and antennas, to enable direct wireless interrogation. Finally, we showcase the seamless integration of the sensor with COTS RFID ICs and WiFi OFDM based backscatter by reading the sensor phase changes via simple channel estimation processes.

\subsection{Miniaturized force sensor design to solve for space constraints}

In order to keep the sensor design optimized for space constraints, we design a capacitative force sensor with dimensions 4mm $\times$ 2mm (Shown in Fig. \ref{fig:sensor_dime}, as compared to a dime).
a simple and mechanically robust force sensor consisting of 3 layers, a soft polymer layer sandwiched between a top and bottom copper layer (Fig \ref{fig:sensor_def}a). 
The total thickness of the sensor is 0.4mm with each of the copper layers having 0.1mm thickness and the ecoflex polymer being 0.2mm thick.
The width and height of the sensor are 4mm and 2mm respectively.
As forces are applied on the top copper layer, the soft polymer layer deforms and brings the two plates closer (Fig \ref{fig:sensor_def}b). 
Hence, the sensor is assumed to sense the transverse forces acting on the top plate with the
bottom plane is assumed to be fixed. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\textwidth]{design/init_figs/des_sens.pdf}
    \caption{Sensor as compared to a dime coin}
    \label{fig:sensor_dime}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/des2.png}
    \caption{Sensor mechanical composition \& deformation under action of force (Comsol multiphysics simulations)}
    \label{fig:sensor_def}
\end{figure}

As the copper layers come closer to each other due to force on the top layer, the sensor impedance would change. 
To characterize this impedance change, we use a FEM simulator (COMSOL Multiphysics 6.0). 
The FEM simulator meshes the sensor design and solves both mechanical equations (concerned with newton laws and elastic modelling, via COMSOL Structural Mechanics module) and circuit analysis equations (maxwell equations and circuit analysis via COMSOL AC/DC module).
Essentially, via COMSOL we can excite the sensor with an AC voltage source and compute the obtained current as effected.
Further, this computation can be done with sensor being under effect of various levels of force with different geometries computed via the mechanical modelling.
Then, by simply taking voltage to current ratio we can obtain the sensor impedance as a function of force:
\begin{equation}
    Z(F_{\text{mag}})=V(F_{\text{mag}})/I(F_{\text{mag}})
\end{equation}
Hence, this allows computation of impedance versus force readings (Fig. \ref{fig:sensor_imped}a). 
Since the resistive component of the impedance is almost 0, and the reactive component is negative, it shows that the sensor is almost purely capacitative.
Since the resistive part if negligible, the sensor is inherently low-power since it is not wasting any available power in resistive dissipation.

Thus, the sensor is akin to a parallel plate capacitor with the two copper plates acting as electrodes and the polymer layer acting similar to dielectric.
Due to force on the sensor, the two electrodes come closer to each other and hence the capacitance increases.
We can then compute the capacitance from reactive part of impedance by 
\begin{equation}
    C(F_{\text{mag}})=1/(\omega~ \text{im}(Z(F_{\text{mag}})))
\end{equation}
where $\omega=2\pi f$ and $f$ is the frequency of operation.
At a 900 MHz frequency, we obtain the capacitance to force curve as shown in Fig. \ref{fig:sensor_imped}b, with the capacitance going from 6.9 to 7.8 pF, as the force on the sensor increases from 0 to 6 N.
More details on the mechanical design can be found in ~\cite{} (Anon. reference).


\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/des1.png}
    \caption{(a) Sensor impedance vs Force, blue is real part red is imaginary part:  At each force level the sensor impedance is almost purely imaginary which indicates capacitative behaviour (b) How the capacitance increases with force}
    \label{fig:sensor_imped}
\end{figure}

\subsection{Making the capacitative sensor work at RF frequencies}
Now, in order to sense the force we need to sense the change in capacitance from the sensor.
There have been previous capacitative force sensor research work which also associating force to capacitance change.
However, they use a CDC (Capacitance to Digital Converter) in order to sense the capacitance.
CDC works in a manner similar to comsol simulation, it excites the sensor with a AC voltage ($\sim$kHz frequency typically) and measures the current to compute impedance and hence the capacitance. So, in order to read the capacitative sensors wirelessly in a batteryless way to respect the energy constraints, we would need a re-design of today's low-power backscatter sensing modalities which come equipped with an ADC but not a CDC.

Here, we show a key insight which actually bypasses this requirement of a dedicated CDC block completely by directly sensing capacitance via RF interrogation.
Say if we have an antenna receiving signals $s$ at RF frequency $\omega$, and a transmission line 50 $\Omega$ matched to $\omega$, and we terminate this with the capacitative sensor (basically like a pure reactive load), as shown in Fig. \ref{fig:sensor_refl}.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/sens_refl.pdf}
    \caption{Reflection coefficient}
    \label{fig:sensor_refl}
\end{figure}

The reflected signals from the capacitor are multiplied by the reflection coefficient $\Gamma$ and then backscattered by the antenna. Notice that due to the purely capacitative nature of the sensor $\Gamma$ has the form of $\frac{a-bj}{a+bj}$ 
and hence can be rewritten in polar form as $\frac{\sqrt{a^2+b^2}e^{-j\tan^{-1}(b/a)}}{\sqrt{a^2+b^2}e^{j\tan^{-1}(b/a)}}$.
Thus, $\Gamma$ has unit magnitude and a phase term $\phi(F_{\text{mag}})$ given by $2 tan^{-1}(b/a)$, which evaluates to

\begin{equation}
\phi(F_{\text{mag}}) = 2 tan^{-1}(1/50\omega C(F_{\text{mag}}))
\label{eq:phase}
\end{equation}

\noindent Hence, the capacitative force sensor when excited by a RF frequency $\omega$ effectively encodes it's capacitance value in the reflected signal phase. Thus, by sensing the reflected phase changes we can estimate the capacitance and hence $F_{\text{mag}}$. This methodology of sensing capacitance directly via RF backscattered phase sensing would total bypasses any requirement of complicated blocks like CDC and allows for integration with existing backscatter implementations as well.
Using Eq. \eqref{eq:phase} and capacitance values from AC/DC Comsol simulations, we observe that the sensor gives about 20$^o$ phase shift when force increases from 0-6 N as shown in Fig. \ref{fig:sensor_bw_sims}b.


% A natural question however is that with a mm-scale sensor, how do we actually excite the sensor with a RF frequency and verify if we get these phase changes as capacitance varies? 
% % In simulations we can very easily connect top copper layer to AC source with frequency $\omega$ and ground the bottom copper layer to evaluate the capacitance
In order to show a practical deployment of Fig. \ref{fig:sensor_refl}, we simulate a PCB with a microstrip line matched to 900 MHz frequency using Comsol RF module\footnote{900 MHz is a popular ISM band which works well for in-body applications and is supported by variety of technologies like EPC RFID and LoRa}. 
The PCB consists of two layers, on the top there is a signal trace which is 2mm wide similar to the sensor and the bottom layer is the ground plane.
The bottom copper plate of the sensor is directly soldered onto the signal trace.
Now, in order to have the sensor and PCB ground common, we use a tungsten wire filament to connect the top copper plate with a small ground pad on the top layer using via (Fig. \ref{fig:sensor_bw_sims} a). This simulation using Comsol RF module can then be linked to Comsol Structural Mechnanics module similar to the previous simulations with AC/DC module.
However, this time Comsol FEM solver solves both structural mechanics equation and maxwell's equation concerned with the RF signal propagation.
The PCB simulations utilize a single lumped port to excite the transmission line, and the sensor phases are hence encoded onto the S11 measurements.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/des_bondwiresims.pdf}
    \caption{PCB sims with RF module: Phase change from RF simulations (blue) are well modelled by the extarpolations from AC/DC simulations (red)}
    \label{fig:sensor_bw_sims}
\end{figure}

We confirm that the S11 phase changes (about 20$^o$ from RF comsol simulations) from the RF module simulations are consistent with the earlier simulations with AC/DC module (Fig. \ref{fig:sensor_bw_sims} b).
Note that the AC/DC module just give capacitance measurements which are mathematically converted to phase via \eqref{eq:phase}, whereas the RF module simulation is a faithful end-to-end FEM simulation which confirms that the sensor can work in a practical form factor. 
The small discrepancies can be addressed due to two facts, first the AC/DC module computes DC capacitance which may not be purely accurate at 900 MHz and further the addition of small bondwire may cause these minor discrepancies.
In Section \ref{sec:implementation} we fabricate this PCB and confirm that the RF module simulations are consistent with the actual implementation.
Hence, we verify that the capacitance change affects the phase shifts and this concept can be utilized to bypass the need of a dedicated CDC block and pave the way for energy, as well as space-optimized wireless capacitative force sensing.

% Here we can write about the bondwire part of the stuff: how to get to phase change essentially
% \begin{equation}
%     \Gamma = \frac{\left(50-\frac{1}{j\omega C(F_{\text{mag}})} \right)}{\left(50+\frac{1}{j\omega C(F_{\text{mag}})} \right)}
% \end{equation}
% $$\phi(F_{\text{mag}}) = \angle\left(\frac{\left(50-\frac{1}{j\omega C(F_{\text{mag}})} \right)}{\left(50+\frac{1}{j\omega C(F_{\text{mag}})} \right)}\right)$$ 


% The important point to make here is that we can do phase change with the sensor acting in a thru mode. We can show S11, S12 simulatiomns here to convince people.

\subsection{Wireless batteryless reading of \name to solve for energy constraints}

Now, we would describe how \name's capacitative sensor can be read wirelessly without a battery to respect the energy constraints.
When a reader situated remotely to the sensor tries to read the reflected signal phases from the sensor, it also needs to isolate the signal from the sensor in order to achieve the same. 
Henceforth, it is required for the sensor phase-shifted signals to also be modulated before they are reflected back.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/sens_modulation.pdf}
    \caption{Placement of sensor modulation block}
    \label{fig:sens_modulation}
\end{figure}

Now we can place a modulation block either before the sensor, or after the sensor as shown in Fig. \ref{fig:sens_modulation}. The key advantage of the earlier approach is that it allows us to use any existing COTS backscatter modulation IC today since these ICs are designed to simply take the signals from antenna, feed it to RF energy harvestor to power up a low-power modulator and reflect the signals back. Hence, if we put the sensor after the modulation block, the signals wont even reach the sensor as the commercial modulation block would reflect the signals off totally. 

It is indeed possible to have the modulation before sensor by designing a custom modulation block, for example it is popular to have a switch toggling at a known frequency to give frequency shifted modulation and that can work in a through mode as shown by a lot of past works \cite{}. But these blocks are not commercialized and making them in a miniaturized form factor to respect the posed space constraints is not straightforward.
On the flip-side, keeping the modulation block after sensor requires the sensor to work in a thru phase shift mode, as opposed to the simple reflection phase shift as discussed in the previous subsection. We will now show how \name sensor design actually achieves this even via thru-mode phase modulation which allows it to integrate with COTS modulation blocks and optimize for both space and energy constraints.
% Thus, to do so, we propose to add a modulation block as shown in Fig. \ref{}. 
% The key idea is that the sensor would add a phase shift given by $\phi(F_{\text{mag}})$ and the modulation block would add certain modulation $m(t)$ to the received signal $s(t)$.
% Thus the sensor+modulation block would backscatter the signal $s(t)m(t)e^{j\phi(F_{\text{mag}})}$. 
% A natural question is, if the sensor encodes phase shift in reflections, shouldn't the  signals from sensor just reflect off and never end up going through the modulation? Hence $s(t)e^{j\phi(F_{\text{mag}})}$ would be the signal getting backscattered instead without any moudlation.


% A naive way to modulate sensor signals is to perform on-off switching modulation. 
% This effectively provides frequency shifts to the reflected signals and thus modulating the signals in effect.
% The reader can read these phase changes at these frequency shifted signals to ascertain the force values.
% This technique is common among various past works \cite{}.
% However, these designs use a clock source for these switches, from a battery-powered source like a low power micro-controller, with the power requirements being a few $\mu$Watts. These can be met via energy harvestor techniques, however as most of these are proof-of-concept research platforms, the energy harvestor integration is left to future work. 

% A key distinguishing feature of \name sensor design is that in addition to these naive switch based methods, \name can simply piggyback on existing UHF RFID backscatter solutions which already integrate energy harvestors and backscatter modulators in a commercial IC package \cite{}. However, the commercial ICs are designed to reflect the modulated signals coming from antenna, and the only place where we can put the sensor is between the antenna and the IC. 
% Hence, if the sensor purely reflects all the signals with a phase shift, the signals will not reach the IC in the first place and thus would just get reflected back unmodulated.
% Thus, a key requirement to enabling this integration with commercially available ICs is that the sensor should not only work in a reflection mode, but also in a thru mode. 
% Large body of past works work only in a reflection mode ~\cite{} and hence do not enjoy this feature of seamless integrability with the existing backscatter technologies. 

To show how \name works in thru mode, we move the sensor in the middle of the PCB simulations (Fig. \ref{fig:sensor_vna_res}) as compared to towards the end as shown in previous subsection. This allows us to define 2 lumped ports, one of each end of the PCB, and by observing S12 phase and magnitude we can verify if the sensor can work in a thru mode. For this simulation we obtain the S12 phase changes and observe that the phase changes are about half the magnitude we had before, that is 10$^{o}$ for 0-6 N forces as compared to 20$^{o}$ before. Now, when we keep the other port as reflective and estimate the S11 phase, we get almost the same phase shifts as before (around 20$^{o}$).

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{results/init_figs/res2.png}
    \caption{Phase doubling effect due to two sided travel via sensor: simulations}
    \label{fig:sensor_vna_res}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/sens_mod_fin.pdf}
    \caption{Placement of sensor modulation block}
    \label{fig:sens_modulation_fin}
\end{figure}

Hence, intuitively what happens is that when a signal $s(t)$ travel through the sensor, it first gets a certain value of phase shift and the sensor passes the signal through $s(t)e^{j\phi(F_{\text{mag}})/2}$. Then, when the signals get modulated $s(t)e^{j\phi(F_{\text{mag}})/2}m(t)$, reflect and pass through the sensor again, the total phase shift doubles up $s(t)e^{j\phi(F_{\text{mag}})}m(t)$ and reaches back to the reflective levels as described in Eqn \eqref{eq:phase}. 
This is visually illustrated in Fig. \ref{fig:sens_modulation_fin}
Thus, the reflected signal has both the modulation component, as well as a phase shift. The wireless reader can use the modulation to isolate the sensor reflections from the environmental reflections and then estimate these phase shifts from the isolated signal.
This process can be any standardized demodulation block to isolate the sensor signals and then from the estimated channel these phase shifts can be computed.
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{implementation/impl.pdf}
    \caption{Interfacing the sensor with RFID tags: 
    % (a) Sensor prototype with two tungsten wire filaments compared to a dime coin 
    (a) Using a tweezer to peel away the RFID IC from the antenna (b) Placing the sensor tungsten wires below the conductive pads for the IC and (c) Final sensor + RFID prototype}
    \label{fig:my_label}
\end{figure*}

\subsection{Putting it all together: \name sensor with COTS RFIDs}

In order to demonstrate wireless, batteryless force sensing we integrate our designed sensor prototype with RFIDs.
RFID technology has matured over the past decade and today there are commercial ICs available ~\cite{} which integrate a full-fledged energy harvestor and modulator logic. We can integrate the sensor with these RFID ICs, as well as COTS available RFIDs via certain fabrication techniques discussed in Section \ref{sec:implementation}. However, in effect, from a design point of view, the sensor is interfaced in parallel to the RFID modulation block, as shown in Fig. \ref{fig:sens_modulation_fin}.
% There has been one past challenge paper \cite{} which motivates integrating temperature, photo and binary touch/no-touch sensors based majorly on change in resistance with RFIDs.
% The major issue with the paper was that integrating resistive sensors with RFIDs lead to reduced range.



Since \name's capacitative force sensor has negligible resistive impedance, it only effects the phases of the signals passing through, and thus the input to the energy harvestor unit is the same magnitude signal as it would have been without the sensor. Hence, \name's method of integration does not adversely affect the RFID reading ranges.



To tie up \name's design, the only component left to describe is the wireless reader.
As explained towards end of previous subsection, \name sensor can use any COTS RFID reader which performs RFID channel estimates.
The COTS RFID reader can identify the signals coming from the sensor via figuring out the EPC id number of the RFID IC integrated with sensor.
Then, the RFID reader can observe the channel estimates of this particular tag and calculate sensor phase jumps to estimate applied forces. 

In order to estimate these phase jumps with COTS readers a challenge is the hopping nature of these COTS readers. As per FCC guidelines the readers need to change their frequencies after every 200 milliseconds to avoid interference with other readers in the environment. Most of the COTS readers introduce a random phase offset due to hopping which could show up in the phase calculations.
However, \name's sensing is robust to these random phase offsets as the phase change introduced by the force appears across each channel as a differential phase jump (Fig. ). Hence, \name calculates the phase jumps at each of the RFID hopping frequencies and then averages them to obtain a very clean phase jump measurement (accurate to about 1$^o$ precision) which can then be used to compute the applied forces from the batteryless miniaturized sensor.
% However, \name operates on self-differential phase instead of absolute phase, that is, to determine the force applied \name estimates the only the change in phase across the , which automatically removes any of these fixed offsets.

% Prior work ~\cite{} puts forward a challenge in achieving the same: it shows how errors in RFID sensing can be substantial. The metrics considered there were phase, RSSI and DMRT: and it was considred how stable these quantities are. However, they didnt tuen off hopping: doing this with hopping could be a challenge. Dont go in this much detail: just tell its a challenge and they didnt consider time differential phase, and WiForce another past work basically relied on OFDM transforms which are not avaialble to RFID?

% in augmenting sensors to RFIDs ended up using series resistors which sense quantities by sensing relative drop in RSSIs of co-located tags. However, this requires presence of a second tag to take reference tag and further series networks are not generalizable (How to design something which notches/whatever DMRS did was to basically terse around RSSI problems via reference tag). But 

% \subsubsection{Single frequency based search}

% \subsubsection{Hopping based algorithm}



% \subsection{How \name integrates seamlessly with any wireless technology}

% Finally, here we can write two things:

% \begin{itemize}
%   \item Reading via switch based OFDM backscatter like we did in WiForce: however counter doppler now
%   \item RFID based stuff which we are doing now
% \end{itemize}


==> design/design_v2.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}
% \textcolor{blue}{
% So the design can really go 2 ways: we go full blown into doppler suppression for RFID and make it a targeted RFID paper, or we put across the various COTS reader arguments. 
% \begin{itemize}
%   \item The prior approach is more well suited for NSDI 
%   \item The former becomes towards maybe Mobisys demo/Sensys. Also we can include real-life bottle sensing etc applications whereas NSDI can be in general
% \end{itemize}
% Main thing to sell here is the sensor and not the RFID stuff, we will kindof just overlook it and write the paper how Omid et al wrote. 
% So kindof makes sense to demonstrate the prior one for now in next 20 days. List of technologies which can be potentially demonstrated:
% 1. RFID (batteryless robot experiment, knee implant)
% 2. OFDM (show some AR/VR applications use WiForce algo)
% 3. LoRA/nb-IoT
% 4. UWB if possible this will make it slam dunk
% }

\name presents the first stickable, wireless and batteryless (mm-scale) force sensors.
\name solves both the energy and space constraints required for wireless force sensing.
In this section we delineate various facets behind \name.
First, we will present the design guidelines to create a capacitative sensor that works at RF frequencies.
Second, we show how this sensor can be integrated with batteryless RFID systems to modulate the backscattered signal from the sensor.
Finally we present the details on how the RFID reader finally isolates the sensor modulated signal and reads the forces wirelessly from the sensor.
% In this section we present the various design facets of \name which enable these features: (1) miniaturized passive , (2) wireless and (3) seamless integrability. 
% First, we explain the sensor design and how it transduces force onto change in impedance. Then, we go into the details on how the sensor can be integrated with RF components, like ICs and antennas, to enable direct wireless interrogation. Finally, we showcase the seamless integration of the sensor with COTS RFID ICs and WiFi OFDM based backscatter by reading the sensor phase changes via simple channel estimation processes.

\subsection{Enabling joint communication+sensing via RF Force capacitor}

The capacitive force sensors are generally fabricated by having two conductive surfaces separated by a soft polymer dielectric.
As force is applied on the capacitor, the polymer deforms and the two conductors get close to each other which increases the capacitance.
Typically, the past work has sensed this increase in capacitance by using extra electronics like Capacitance to Digital Converters (CDC) which sense capacitance by sensing the charge accumulation on the conductive plates.
However, none of the batteryless RFID systems today feature a CDC and thus capacitive force sensors can not be interfaced.
Further the CDCs are power hungry, since in order to sense these charge accumulation they need to excite the capacitor with an AC voltage and then measure the charge response.
Doing this with the stringent power requirements of batteryless RFID systems working with RF harvested power would not be trivial and might even require a re-design of existing systems to incorporate capacitve sensors.
In \name we bypass these extra digital electronics requirements by proposing a joint communication sensing approach with force sensitive capacitors by motivating the fact that capacitance change can be sensed via direct analog RF interrogation.

The key insight \name has to allow for joint communication sensing is that capacitance change can also be associated to change in RF phase, when interrogated directly with RF frequency signals. This is akin to how varactors produce continuous phase shifts by tuning the capacitance\cite{}. In case of a force sensitive capacitor, the capacitance is a function of force applied on it, represented as $C(F_{\text{mag}})$.
Say if we have an antenna receiving signals $s$ at RF frequency $\omega$, and a transmission line 50 $\Omega$ matched to $\omega$, and we terminate this with the capacitative sensor (basically like a pure reactive load), as shown in Fig. \ref{fig:sensor_refl}.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/sens_refl.pdf}
    \caption{Reflection coefficient}
    \label{fig:sensor_refl}
\end{figure}

The reflected signals from the capacitor are multiplied by the reflection coefficient $\Gamma$ and then backscattered by the antenna. Notice that due to the purely capacitative nature of the sensor $\Gamma$ has the form of $\frac{a-bj}{a+bj}$ 
and hence can be rewritten in polar form as $\frac{\sqrt{a^2+b^2}e^{-j\tan^{-1}(b/a)}}{\sqrt{a^2+b^2}e^{j\tan^{-1}(b/a)}}$.
Thus, $\Gamma$ has unit magnitude and a phase term $\phi(F_{\text{mag}})$ given by $2 tan^{-1}(b/a)$, which evaluates to

\begin{equation}
\phi(F_{\text{mag}}) = 2 tan^{-1}(1/50\omega C(F_{\text{mag}}))
\label{eq:phase}
\end{equation}

Hence, the capacitance increases as the force applied on it increases, and this leads to a change in reflected signal phase when interrogated at an RF frequency $\omega$, as described by the equation \eqref{eq:phase}.

% In order to keep the sensor design optimized for space constraints, we design a capacitative force sensor with dimensions 4mm $\times$ 2mm (Shown in Fig. \ref{fig:sensor_dime}, as compared to a dime).
% a simple and mechanically robust force sensor consisting of 3 layers, a soft polymer layer sandwiched between a top and bottom copper layer (Fig \ref{fig:sensor_def}a). 
% The total thickness of the sensor is 0.4mm with each of the copper layers having 0.1mm thickness and the ecoflex polymer being 0.2mm thick.
% The width and height of the sensor are 4mm and 2mm respectively.
% As forces are applied on the top copper layer, the soft polymer layer deforms and brings the two plates closer (Fig \ref{fig:sensor_def}b). 
% Hence, the sensor is assumed to sense the transverse forces acting on the top plate with the
% bottom plane is assumed to be fixed. 

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.3\textwidth]{design/init_figs/des_sens.pdf}
%     \caption{Sensor as compared to a dime coin}
%     \label{fig:sensor_dime}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{design/init_figs/des2.png}
%     \caption{Sensor mechanical composition \& deformation under action of force (Comsol multiphysics simulations)}
%     \label{fig:sensor_def}
% \end{figure}

% As the copper layers come closer to each other due to force on the top layer, the sensor impedance would change. 
% To characterize this impedance change, we use a FEM simulator (COMSOL Multiphysics 6.0). 
% The FEM simulator meshes the sensor design and solves both mechanical equations (concerned with newton laws and elastic modelling, via COMSOL Structural Mechanics module) and circuit analysis equations (maxwell equations and circuit analysis via COMSOL AC/DC module).
% Essentially, via COMSOL we can excite the sensor with an AC voltage source and compute the obtained current as effected.
% Further, this computation can be done with sensor being under effect of various levels of force with different geometries computed via the mechanical modelling.
% Then, by simply taking voltage to current ratio we can obtain the sensor impedance as a function of force:
% \begin{equation}
%     Z(F_{\text{mag}})=V(F_{\text{mag}})/I(F_{\text{mag}})
% \end{equation}
% Hence, this allows computation of impedance versus force readings (Fig. \ref{fig:sensor_imped}a). 
% Since the resistive component of the impedance is almost 0, and the reactive component is negative, it shows that the sensor is almost purely capacitative.
% Since the resistive part if negligible, the sensor is inherently low-power since it is not wasting any available power in resistive dissipation.

% Thus, the sensor is akin to a parallel plate capacitor with the two copper plates acting as electrodes and the polymer layer acting similar to dielectric.
% Due to force on the sensor, the two electrodes come closer to each other and hence the capacitance increases.
% We can then compute the capacitance from reactive part of impedance by 
% \begin{equation}
%     C(F_{\text{mag}})=1/(\omega~ \text{im}(Z(F_{\text{mag}})))
% \end{equation}
% where $\omega=2\pi f$ and $f$ is the frequency of operation.
% At a 900 MHz frequency, we obtain the capacitance to force curve as shown in Fig. \ref{fig:sensor_imped}b, with the capacitance going from 6.9 to 7.8 pF, as the force on the sensor increases from 0 to 6 N.
% More details on the mechanical design can be found in ~\cite{} (Anon. reference).


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{design/init_figs/des1.png}
%     \caption{(a) Sensor impedance vs Force, blue is real part red is imaginary part:  At each force level the sensor impedance is almost purely imaginary which indicates capacitative behaviour (b) How the capacitance increases with force}
%     \label{fig:sensor_imped}
% \end{figure}


For the past work, which use a capacitor at low frequencies (a few kHz) and sense the capacitance by sensing the charge accumulation via the CDC, the sensor sensitivity and performance improves as the capacitance increases.
This is because the charge accumalation, $Q_{\text{accumulated}}=C(F_{\text{mag}})V_{\text{applied}}$ is directly related to capacitance, and thus it is favorable to design sensors with higher capacitances, and a common design theme is to have higher dielectric constant polymers or higher area conductors.
However, unlike the low frequency counterparts, RF force capacitors are to be read via phase changes, and the quantity of interest is the total phase change due to the maximum permissible force for the sensor $F_{\text{max}}$, and $C_0$ is the nominal capacitance of the sensor at $0$ N force:
\begin{equation}
\Delta \phi = 2 tan^{-1}(1/50\omega C(F_{\text{max}}))-2 tan^{-1}(1/50\omega C_0))
\label{eqn:delphi}
\end{equation}
To get the best sensitiveness, we need to design the capacitance such that $\Delta \phi$ is maximized for the operating frequency $\omega$.
In comparison to charge accumulation, which is a simple linear relationship, $\Delta \phi$ has the non-linear arctan function which does not make the sensor design as straightforward as maximizing capacitance.
To understand the design choice behind RF Force capacitor, we plot $\Delta \phi$  in Fig. \ref{fig:delphi} for an empirical relationship between $C(F_{\text{max}})=1.75*C_0$, (i.e. $\frac{\Delta C}{C_0}$=0.75, a common operating point of the capacitive sensors), and different ranges of $C_0$ values.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{design/init_figs/cap_motiv.pdf}
    \caption{How different values of $C_0$ affect $\Delta \phi$}
    \label{fig:delphi}
\end{figure}

We observe from Fig. \ref{fig:delphi} that for $C_0 = 0.1$ pF, $100$ pF the total phase change achievable at the 900 MHz\footnote{900 MHz is a popular ISM band which works well for in-body applications and is supported by variety of technologies like EPC RFID and LoRa} frequency of interest would be $<5^{o}$ which is not a good operating point.
Intuitively what is happening is that \eqref{eqn:delphi} has the arctan function, which saturates as the input gets closer to both $0$ and $\infty$, and hence at $\omega \to 0$, the total phase changes are negligible as the input is driven to $\infty$ and at high $C_0 \omega \to \infty$ the input goes to $0$ and that also gives lesser phase changes.
Hence, RF force capacitor can not just maximize the capacitance blindly and has to be designed at reasonable nominal capacitances.
We get reasonable phase changes $>15^{o}$ for $C_0 = 1,10$ pF so the ideal operating point of the sensor is to get the nominal capacitance within this range.
Hence, a natural question is how can we design the sensors such that nominal capacitances fall in the required ranges such that the phase change effect is appreciable enough.

\subsection{Design of RF Force Capacitor}
% A natural question however is that with a mm-scale sensor, how do we actually excite the sensor with a RF frequency and verify if we get these phase changes as capacitance varies? 
% % In simulations we can very easily connect top copper layer to AC source with frequency $\omega$ and ground the bottom copper layer to evaluate the capacitance
Now, to get sufficient phase changes at 900 MHz RF frequencies, we need to design a capacitor with nominal capacitance being of the order of 1-10 pF.
Further, in order to compute the exact $\Delta \phi$ we also need to compute $C(F_{\text{max}})$ and not the empirical relationship as in previous subsection.
In order to do so, we need to solve both the structural mechanics equations to compute the polymer deformation and then feed the deformed geometry to maxwell equations to compute the effective capacitance of the sensor and hence obtain the $\Delta \phi$ metric.

Since the polymer deformation has a non-linear stress-strain relationship, and the maxwells equations are not straightforward to be solved in an analytic closed form approach, we utilize FEM simulation framework, Comsol Multiphysics 6.0 to simulate the sensor capacitive effect. The software takes the sensor geometry as an input and meshes the geometry to form small elements where the differential equations can be solved numerically and final results are then collated across each mesh element's solution.
However, even with the Comsol framework, obtaining capacitance at RF frequencies is challenging, since as RF frequencies typically the available parameters are the S-parameters which include the phase and magnitude of RF signal excitation. 
Hence, we can directly obtain the RF phase change matrix $\Delta \phi$ at RF but not capacitance.
At lower frequencies, Comsol reports current and voltage measurements which allows us to compute $C(F_{\text{mag}})$. 
Then from \eqref{eq:phase} we can compute phase by assuming capacitance values remain similar at RF frequencies.
To justify that the two simulations are more or less consistent we compare the final phase results from both and show they are close to each ther. 

In order to keep the sensor design optimized for space constraints of mm-scale, we design the capacitative force sensor with dimensions 4mm $\times$ 2mm (Shown in Fig. \ref{fig:sensor_dime}, as compared to a dime).
The sensor consists of 3 layers, a soft polymer layer sandwiched between a top and bottom copper layer (Fig \ref{fig:sensor_def}a). 
The total thickness of the sensor is 0.4mm with each of the copper layers having 0.1mm thickness and the ecoflex polymer being 0.2mm thick.
The width and height of the sensor are 4mm and 2mm respectively.
As forces are applied on the top copper layer, the soft polymer layer deforms and brings the two plates closer (Fig \ref{fig:sensor_def}b), which increases the sensor capacitance. 
Hence, the sensor is assumed to sense the transverse forces acting on the top plate with the
bottom plate is assumed to be fixed. 

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.3\textwidth]{design/init_figs/des_sens.pdf}
%     \caption{Sensor as compared to a dime coin}
%     \label{fig:sensor_dime}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/des2.png}
    \caption{Sensor mechanical composition \& deformation under action of force (Comsol multiphysics simulations)}
    \label{fig:sensor_def}
\end{figure}

We use COMSOL Structural Mechanics module for the non-linear elastic modelling of the polymer layer and 
via COMSOL AC/DC module we can excite the sensor with an AC voltage source and compute the obtained current as effected.
This computation can be done with sensor being under effect of various levels of force applied on the sensor.
Then, by simply taking voltage to current ratio we can obtain the sensor impedance as a function of force:
\begin{equation}
    Z(F_{\text{mag}})=V(F_{\text{mag}})/I(F_{\text{mag}})
\end{equation}
Hence, this allows computation of sensor impedance versus force readings (Fig. \ref{fig:sensor_imped}a). 
Since the resistive component of the impedance is almost 0, and the reactive component is negative, it shows that the sensor is almost purely capacitative.
We obtain the capacitance to force curve as shown in Fig. \ref{fig:sensor_imped}b, with the capacitance going from 1 to 1.75 pF, as the force on the sensor increases from 0 to 6 N.
This meets our target of sensor design with nominal capacitance about 1 pF.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/cap_v_force.pdf}
    \caption{(a) Sensor impedance vs Force:  At each force level the sensor impedance is almost purely imaginary which indicates capacitative behaviour (b) How the capacitance increases with force}
    \label{fig:sensor_imped}
\end{figure}

However, these simulations assume the low-frequency capacitance value to extrapolate and work similarly at RF frequencies, and we need to verify this approximation.
Now, in order to both verify this effect at RF frequencies, we simulate the sensor attached to a PCB with a microstrip line matched to 900 MHz frequency using COMSOL RF module. 
Basically, this PCB implements a transmission line which has the capacitive sensors as the termination load, in a way it practically implements Fig. \ref{fig:sensor_refl}.
The PCB consists of two layers, on the top there is a signal trace which is 2mm wide similar to the sensor and the bottom layer is the ground plane.
The bottom copper plate of the sensor is directly soldered onto the signal trace.
Now, in order to have the sensor and PCB ground common, we use a tungsten wire filament to connect the top copper plate with a small ground pad on the top layer using via (Fig. \ref{fig:sensor_bw_sims} a). This simulation using Comsol RF module can then be linked to Comsol Structural Mechnanics module similar to the previous simulations with AC/DC module.
However, this time Comsol FEM solver solves both structural mechanics equation and maxwell's equation concerned with the RF signal propagation.
The PCB simulations utilize a single lumped port to excite the transmission line, and the sensor phases are hence encoded onto the S11 measurements.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/des_bondwiresims.pdf}
    \caption{PCB sims with RF module: Phase change from RF simulations (blue) are well modelled by the extarpolations from AC/DC simulations (red)}
    \label{fig:sensor_bw_sims}
\end{figure}

We confirm that the S11 phase changes (about 20$^o$ from RF comsol simulations) from the RF module simulations are consistent with the earlier simulations with AC/DC module (Fig. \ref{fig:sensor_bw_sims} b).
Note that the AC/DC module just give capacitance measurements which are mathematically converted to phase via \eqref{eq:phase}, whereas the RF module simulation is a faithful end-to-end FEM simulation which confirms that the sensor can work in a practical form factor. 
The small discrepancies can be attributed to two facts. First the AC/DC module computes DC capacitance which may not be purely accurate at 900 MHz and further the addition of small tungsten filament may also cause some additional minor discrepancies.
In Section \ref{sec:implementation} we fabricate this PCB and confirm that the RF module simulations are consistent with the actual implementation.
Hence, we verify that the capacitance change affects the phase shifts and this concept can be utilized to interrogate the sensor directly at RF frequencies and thus paves the way for energy, as well as space-optimized wireless capacitative force sensing.



% Here we can write about the bondwire part of the stuff: how to get to phase change essentially
% \begin{equation}
%     \Gamma = \frac{\left(50-\frac{1}{j\omega C(F_{\text{mag}})} \right)}{\left(50+\frac{1}{j\omega C(F_{\text{mag}})} \right)}
% \end{equation}
% $$\phi(F_{\text{mag}}) = \angle\left(\frac{\left(50-\frac{1}{j\omega C(F_{\text{mag}})} \right)}{\left(50+\frac{1}{j\omega C(F_{\text{mag}})} \right)}\right)$$ 


% The important point to make here is that we can do phase change with the sensor acting in a thru mode. We can show S11, S12 simulatiomns here to convince people.

\subsection{Wireless batteryless reading of \name to solve for energy constraints}

Now, we would describe how \name's capacitative sensor can be read wirelessly without a battery to respect the energy constraints.
When a reader situated remotely to the sensor tries to read the reflected signal phases from the sensor, it also needs to isolate the signal from the sensor in order to achieve the same. 
Henceforth, it is required for the sensor phase-shifted signals to also be modulated before they are reflected back.
However, in order to add the modulation block, it is required that the sensor also passes the signals through instead of just reflecting it back, as discussed in the previous subsection. We will now show how \name sensor design actually achieves thru-mode phase modulation which allows it to integrate with modulation blocks.

To show how \name works in thru mode, we move the sensor in the middle of the PCB simulations (Fig. \ref{fig:sensor_vna_res}) as compared to towards the end as shown in previous subsection. This allows us to define 2 lumped ports, one of each end of the PCB, and by observing S12 phase and magnitude we can verify if the sensor can work in a thru mode. For this simulation we obtain the S12 phase changes and observe that the phase changes are about half the magnitude we had before, that is 10$^{o}$ for 0-6 N forces as compared to 20$^{o}$ before. Now, when we keep the other port as reflective and estimate the S11 phase, we get almost the same phase shifts as before (around 20$^{o}$).

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{results/init_figs/thruPCB_sims.pdf}
    \caption{Phase doubling effect due to two sided travel via sensor: simulations}
    \label{fig:sensor_vna_res}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/sens_mod_fin.pdf}
    \caption{Placement of sensor modulation block}
    \label{fig:sens_modulation_fin}
\end{figure}

Hence, intuitively what happens is that when a signal $s(t)$ travel through the sensor, it first gets a certain value of phase shift and the sensor passes the signal through $s(t)e^{j\phi(F_{\text{mag}})/2}$. Then, when the signals get modulated $s(t)e^{j\phi(F_{\text{mag}})/2}m(t)$, reflect and pass through the sensor again, the total phase shift doubles up $s(t)e^{j\phi(F_{\text{mag}})}m(t)$ and reaches back to the reflective levels as described in Eqn \eqref{eq:phase}. 
This is visually illustrated in Fig. \ref{fig:sens_modulation_fin}
Thus, the reflected signal has both the modulation component, as well as a phase shift. 
The wireless reader can use the modulation to isolate the sensor reflections from the environmental reflections and then estimate these phase shifts from the isolated signal.
This can be done by using any standardized demodulation block to isolate the sensor signals and then from the estimated channel these phase shifts can be computed.
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{implementation/impl.pdf}
    \caption{Interfacing the sensor with RFID tags: 
    % (a) Sensor prototype with two tungsten wire filaments compared to a dime coin 
    (a) Using a tweezer to peel away the RFID IC from the antenna (b) Placing the sensor tungsten wires below the conductive pads for the IC and (c) Final sensor + RFID prototype}
    \label{fig:my_label}
\end{figure*}

\subsection{Putting it all together: \name sensor with COTS RFIDs}

In order to demonstrate wireless, batteryless force sensing we integrate our designed sensor prototype with RFIDs.
RFID technology has matured over the past decade and today there are commercial ICs available ~\cite{} which integrate a full-fledged energy harvestor and modulator logic. We can integrate the sensor with these RFID ICs, as well as COTS available RFIDs via certain fabrication techniques discussed in Section \ref{sec:implementation}. However, in effect, from a design point of view, the sensor is interfaced in parallel to the RFID modulation block, as shown in Fig. \ref{fig:sens_modulation_fin}.
% There has been one past challenge paper \cite{} which motivates integrating temperature, photo and binary touch/no-touch sensors based majorly on change in resistance with RFIDs.
% The major issue with the paper was that integrating resistive sensors with RFIDs lead to reduced range.



Since \name's capacitative force sensor has negligible resistive impedance, it only effects the phases of the signals passing through, and thus the input to the energy harvestor unit is the same magnitude signal as it would have been without the sensor. Hence, \name's method of integration does not adversely affect the RFID reading ranges.



To tie up \name's design, the only component left to describe is the wireless reader.
As explained towards end of previous subsection, \name sensor can use any COTS RFID reader which performs RFID channel estimates.
The COTS RFID reader can identify the signals coming from the sensor via figuring out the EPC id number of the RFID IC integrated with sensor.
Then, the RFID reader can observe the channel estimates of this particular tag and calculate sensor phase jumps to estimate applied forces. 

In order to estimate these phase jumps with COTS readers a challenge is the hopping nature of these COTS readers. As per FCC guidelines the readers need to change their frequencies after every 200 milliseconds to avoid interference with other readers in the environment. Most of the COTS readers introduce a random phase offset due to hopping which could show up in the phase calculations.
However, \name's sensing is robust to these random phase offsets as the phase change introduced by the force appears across each channel as a differential phase jump (Fig. ). Hence, \name calculates the phase jumps at each of the RFID hopping frequencies and then averages them to obtain a very clean phase jump measurement (to about 1$^o$ precision) which can then be used to compute the applied forces from the batteryless miniaturized sensor.
% However, \name operates on self-differential phase instead of absolute phase, that is, to determine the force applied \name estimates the only the change in phase across the , which automatically removes any of these fixed offsets.

% Prior work ~\cite{} puts forward a challenge in achieving the same: it shows how errors in RFID sensing can be substantial. The metrics considered there were phase, RSSI and DMRT: and it was considred how stable these quantities are. However, they didnt tuen off hopping: doing this with hopping could be a challenge. Dont go in this much detail: just tell its a challenge and they didnt consider time differential phase, and WiForce another past work basically relied on OFDM transforms which are not avaialble to RFID?

% in augmenting sensors to RFIDs ended up using series resistors which sense quantities by sensing relative drop in RSSIs of co-located tags. However, this requires presence of a second tag to take reference tag and further series networks are not generalizable (How to design something which notches/whatever DMRS did was to basically terse around RSSI problems via reference tag). But 

% \subsubsection{Single frequency based search}

% \subsubsection{Hopping based algorithm}



% \subsection{How \name integrates seamlessly with any wireless technology}

% Finally, here we can write two things:

% \begin{itemize}
%   \item Reading via switch based OFDM backscatter like we did in WiForce: however counter doppler now
%   \item RFID based stuff which we are doing now
% \end{itemize}


==> design/design_v3_old.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}

\name presents the first stickable, wireless and batteryless (mm-scale) force sensors.
In this section we delineate various facets behind \name.
First, we will present the mm-scale \name sensor design, which is just 0.4mm thick and devoid of any air-gaps allowing for stickable form factor.
The sensor essentially behaves akin to a force variable capacitor (varactor), and thus creates phase shifts in the channel similar to RF varactors.
We analyze this transduction mechanism and profile the capacitance values required to create sufficient phase shifts for fine-grained force sensing.
Going ahead, we show how the force varactor can be interfaced with RFID ICs to modulate these phase shifts for robust wireless sensing.
Finally we present the details on how an externally located RFID reader finally isolates the sensor modulated signal and reads the forces wirelessly from the sensor.

\subsection{\name's mm-scale sensor design and transduction mechanism}

\begin{itemize}
    \item \textbf{Describe the sensor and it's components }
    \item \textbf{Justify the claim of the sensor being a capacitive sensor}
    \item \textbf{Describe the increase in capacitance effect and very slowly get till the arctan equation}
    \item \textbf{This subsection ends with setting up 1-10 pF capacitance requirement which would be met via simulations}
\end{itemize}
The capacitive force sensors are generally fabricated by having two conductive surfaces separated by a soft polymer dielectric.
As force is applied on the capacitor, the polymer deforms and the two conductors get close to each other which increases the capacitance.
Typically, the past work has sensed this increase in capacitance by using extra electronics like Capacitance to Digital Converters (CDC) which sense capacitance by sensing the charge accumulation on the conductive plates.
However, none of the batteryless RFID systems today feature a CDC and thus capacitive force sensors can not be interfaced.
Further the CDCs are power hungry, since in order to sense these charge accumulation they need to excite the capacitor with an AC voltage and then measure the charge response.
Doing this with the stringent power requirements of batteryless RFID systems working with RF harvested power would not be trivial and might even require a re-design of existing systems to incorporate capacitve sensors.
In \name we bypass these extra digital electronics requirements by proposing a joint communication sensing approach with force sensitive capacitors by motivating the fact that capacitance change can be sensed via direct analog RF interrogation.

The key insight \name has to allow for joint communication sensing is that capacitance change can also be associated to change in RF phase, when interrogated directly with RF frequency signals. This is akin to how varactors produce continuous phase shifts by tuning the capacitance\cite{}. In case of a force sensitive capacitor, the capacitance is a function of force applied on it, represented as $C(F_{\text{mag}})$.
Say if we have an antenna receiving signals $s$ at RF frequency $\omega$, and a transmission line 50 $\Omega$ matched to $\omega$, and we terminate this with the capacitative sensor (basically like a pure reactive load), as shown in Fig. \ref{fig:sensor_refl}.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/sens_refl.pdf}
    \caption{Reflection coefficient}
    \label{fig:sensor_refl}
\end{figure}

The reflected signals from the capacitor are multiplied by the reflection coefficient $\Gamma$ and then backscattered by the antenna. Notice that due to the purely capacitative nature of the sensor $\Gamma$ has the form of $\frac{a-bj}{a+bj}$ 
and hence can be rewritten in polar form as $\frac{\sqrt{a^2+b^2}e^{-j\tan^{-1}(b/a)}}{\sqrt{a^2+b^2}e^{j\tan^{-1}(b/a)}}$.
Thus, $\Gamma$ has unit magnitude and a phase term $\phi(F_{\text{mag}})$ given by $2 tan^{-1}(b/a)$, which evaluates to

\begin{equation}
\phi(F_{\text{mag}}) = 2 tan^{-1}(1/50\omega C(F_{\text{mag}}))
\label{eq:phase}
\end{equation}

Hence, the capacitance increases as the force applied on it increases, and this leads to a change in reflected signal phase when interrogated at an RF frequency $\omega$, as described by the equation \eqref{eq:phase}.


For the past work, which use a capacitor at low frequencies (a few kHz) and sense the capacitance by sensing the charge accumulation via the CDC, the sensor sensitivity and performance improves as the capacitance increases.
This is because the charge accumalation, $Q_{\text{accumulated}}=C(F_{\text{mag}})V_{\text{applied}}$ is directly related to capacitance, and thus it is favorable to design sensors with higher capacitances, and a common design theme is to have higher dielectric constant polymers or higher area conductors.
However, unlike the low frequency counterparts, RF force capacitors are to be read via phase changes, and the quantity of interest is the total phase change due to the maximum permissible force for the sensor $F_{\text{max}}$, and $C_0$ is the nominal capacitance of the sensor at $0$ N force:
\begin{equation}
\Delta \phi = 2 tan^{-1}(1/50\omega C(F_{\text{max}}))-2 tan^{-1}(1/50\omega C_0))
\label{eqn:delphi}
\end{equation}
To get the best sensitiveness, we need to design the capacitance such that $\Delta \phi$ is maximized for the operating frequency $\omega$.
In comparison to charge accumulation, which is a simple linear relationship, $\Delta \phi$ has the non-linear arctan function which does not make the sensor design as straightforward as maximizing capacitance.
To understand the design choice behind RF Force capacitor, we plot $\Delta \phi$  in Fig. \ref{fig:delphi} for an empirical relationship between $C(F_{\text{max}})=1.75*C_0$, (i.e. $\frac{\Delta C}{C_0}$=0.75, a common operating point of the capacitive sensors), and different ranges of $C_0$ values.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{design/init_figs/cap_motiv.pdf}
    \caption{How different values of $C_0$ affect $\Delta \phi$}
    \label{fig:delphi}
\end{figure}

We observe from Fig. \ref{fig:delphi} that for $C_0 = 0.1$ pF, $100$ pF the total phase change achievable at the 900 MHz\footnote{900 MHz is a popular ISM band which works well for in-body applications and is supported by variety of technologies like EPC RFID and LoRa} frequency of interest would be $<5^{o}$ which is not a good operating point.
Intuitively what is happening is that \eqref{eqn:delphi} has the arctan function, which saturates as the input gets closer to both $0$ and $\infty$, and hence at $\omega \to 0$, the total phase changes are negligible as the input is driven to $\infty$ and at high $C_0 \omega \to \infty$ the input goes to $0$ and that also gives lesser phase changes.
Hence, RF force capacitor can not just maximize the capacitance blindly and has to be designed at reasonable nominal capacitances.
We get reasonable phase changes $>15^{o}$ for $C_0 = 1,10$ pF so the ideal operating point of the sensor is to get the nominal capacitance within this range.
Hence, a natural question is how can we design the sensors such that nominal capacitances fall in the required ranges such that the phase change effect is appreciable enough.

\subsection{Multiphysics simulation for \name sensor design}
\begin{itemize}
    \item Carefully set up the problem: getting capacitance is not simply $A\epsilon/d$ and requires solving maxwell+structrual mechanics equation
    \item This is where comsol solver steps in. Show the AC/DC simulations here 
    \item This section ends with asking the modulation question to allow for wireless reading and how to interface the sensor with actual components
\end{itemize}
% A natural question however is that with a mm-scale sensor, how do we actually excite the sensor with a RF frequency and verify if we get these phase changes as capacitance varies? 
% % In simulations we can very easily connect top copper layer to AC source with frequency $\omega$ and ground the bottom copper layer to evaluate the capacitance
Now, to get sufficient phase changes at 900 MHz RF frequencies, we need to design a capacitor with nominal capacitance being of the order of 1-10 pF.
Further, in order to compute the exact $\Delta \phi$ we also need to compute $C(F_{\text{max}})$ and not the empirical relationship as in previous subsection.
In order to do so, we need to solve both the structural mechanics equations to compute the polymer deformation and then feed the deformed geometry to maxwell equations to compute the effective capacitance of the sensor and hence obtain the $\Delta \phi$ metric.

Since the polymer deformation has a non-linear stress-strain relationship, and the maxwells equations are not straightforward to be solved in an analytic closed form approach, we utilize FEM simulation framework, Comsol Multiphysics 6.0 to simulate the sensor capacitive effect. The software takes the sensor geometry as an input and meshes the geometry to form small elements where the differential equations can be solved numerically and final results are then collated across each mesh element's solution.
However, even with the Comsol framework, obtaining capacitance at RF frequencies is challenging, since as RF frequencies typically the available parameters are the S-parameters which include the phase and magnitude of RF signal excitation. 
Hence, we can directly obtain the RF phase change matrix $\Delta \phi$ at RF but not capacitance.
At lower frequencies, Comsol reports current and voltage measurements which allows us to compute $C(F_{\text{mag}})$. 
Then from \eqref{eq:phase} we can compute phase by assuming capacitance values remain similar at RF frequencies.
To justify that the two simulations are more or less consistent we compare the final phase results from both and show they are close to each ther. 

In order to keep the sensor design optimized for space constraints of mm-scale, we design the capacitative force sensor with dimensions 4mm $\times$ 2mm (Shown in Fig. \ref{fig:sensor_dime}, as compared to a dime).
The sensor consists of 3 layers, a soft polymer layer sandwiched between a top and bottom copper layer (Fig \ref{fig:sensor_def}a). 
The total thickness of the sensor is 0.4mm with each of the copper layers having 0.1mm thickness and the ecoflex polymer being 0.2mm thick.
The width and height of the sensor are 4mm and 2mm respectively.
As forces are applied on the top copper layer, the soft polymer layer deforms and brings the two plates closer (Fig \ref{fig:sensor_def}b), which increases the sensor capacitance. 
Hence, the sensor is assumed to sense the transverse forces acting on the top plate with the
bottom plate is assumed to be fixed. 

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.3\textwidth]{design/init_figs/des_sens.pdf}
%     \caption{Sensor as compared to a dime coin}
%     \label{fig:sensor_dime}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/des2.png}
    \caption{Sensor mechanical composition \& deformation under action of force (Comsol multiphysics simulations)}
    \label{fig:sensor_def}
\end{figure}

We use COMSOL Structural Mechanics module for the non-linear elastic modelling of the polymer layer and 
via COMSOL AC/DC module we can excite the sensor with an AC voltage source and compute the obtained current as effected.
This computation can be done with sensor being under effect of various levels of force applied on the sensor.
Then, by simply taking voltage to current ratio we can obtain the sensor impedance as a function of force:
\begin{equation}
    Z(F_{\text{mag}})=V(F_{\text{mag}})/I(F_{\text{mag}})
\end{equation}
Hence, this allows computation of sensor impedance versus force readings (Fig. \ref{fig:sensor_imped}a). 
Since the resistive component of the impedance is almost 0, and the reactive component is negative, it shows that the sensor is almost purely capacitative.
We obtain the capacitance to force curve as shown in Fig. \ref{fig:sensor_imped}b, with the capacitance going from 1 to 1.75 pF, as the force on the sensor increases from 0 to 6 N.
This meets our target of sensor design with nominal capacitance about 1 pF.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/cap_v_force.pdf}
    \caption{(a) Sensor impedance vs Force:  At each force level the sensor impedance is almost purely imaginary which indicates capacitative behaviour (b) How the capacitance increases with force}
    \label{fig:sensor_imped}
\end{figure}

However, these simulations assume the low-frequency capacitance value to extrapolate and work similarly at RF frequencies, and we need to verify this approximation.
Now, in order to both verify this effect at RF frequencies, we simulate the sensor attached to a PCB with a microstrip line matched to 900 MHz frequency using COMSOL RF module. 
Basically, this PCB implements a transmission line which has the capacitive sensors as the termination load, in a way it practically implements Fig. \ref{fig:sensor_refl}.
The PCB consists of two layers, on the top there is a signal trace which is 2mm wide similar to the sensor and the bottom layer is the ground plane.
The bottom copper plate of the sensor is directly soldered onto the signal trace.
Now, in order to have the sensor and PCB ground common, we use a tungsten wire filament to connect the top copper plate with a small ground pad on the top layer using via (Fig. \ref{fig:sensor_bw_sims} a). This simulation using Comsol RF module can then be linked to Comsol Structural Mechnanics module similar to the previous simulations with AC/DC module.
However, this time Comsol FEM solver solves both structural mechanics equation and maxwell's equation concerned with the RF signal propagation.
The PCB simulations utilize a single lumped port to excite the transmission line, and the sensor phases are hence encoded onto the S11 measurements.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/des_bondwiresims.pdf}
    \caption{PCB sims with RF module: Phase change from RF simulations (blue) are well modelled by the extarpolations from AC/DC simulations (red)}
    \label{fig:sensor_bw_sims}
\end{figure}

We confirm that the S11 phase changes (about 20$^o$ from RF comsol simulations) from the RF module simulations are consistent with the earlier simulations with AC/DC module (Fig. \ref{fig:sensor_bw_sims} b).
Note that the AC/DC module just give capacitance measurements which are mathematically converted to phase via \eqref{eq:phase}, whereas the RF module simulation is a faithful end-to-end FEM simulation which confirms that the sensor can work in a practical form factor. 
The small discrepancies can be attributed to two facts. First the AC/DC module computes DC capacitance which may not be purely accurate at 900 MHz and further the addition of small tungsten filament may also cause some additional minor discrepancies.
In Section \ref{sec:implementation} we fabricate this PCB and confirm that the RF module simulations are consistent with the actual implementation.
Hence, we verify that the capacitance change affects the phase shifts and this concept can be utilized to interrogate the sensor directly at RF frequencies and thus paves the way for energy, as well as space-optimized wireless capacitative force sensing.



% Here we can write about the bondwire part of the stuff: how to get to phase change essentially
% \begin{equation}
%     \Gamma = \frac{\left(50-\frac{1}{j\omega C(F_{\text{mag}})} \right)}{\left(50+\frac{1}{j\omega C(F_{\text{mag}})} \right)}
% \end{equation}
% $$\phi(F_{\text{mag}}) = \angle\left(\frac{\left(50-\frac{1}{j\omega C(F_{\text{mag}})} \right)}{\left(50+\frac{1}{j\omega C(F_{\text{mag}})} \right)}\right)$$ 


% The important point to make here is that we can do phase change with the sensor acting in a thru mode. We can show S11, S12 simulatiomns here to convince people.

\subsection{Interfacing \name sensor to RFID IC's}

\begin{itemize}
    \item \textbf{The biggest trick allowing us to interface the sensor is the tungsten filaments. So hype up the problem and then inroduce the solution via PCB sims}
    \item \textbf{Show how varactor design gives phase change in thru mode in the PCB sims}
    \item \textbf{Justify the  niceness of tungsten wire as we get performance close to w/o tungsten wire}
\end{itemize}
Now, we would describe how \name's capacitative sensor can be read wirelessly without a battery to respect the energy constraints.
When a reader situated remotely to the sensor tries to read the reflected signal phases from the sensor, it also needs to isolate the signal from the sensor in order to achieve the same. 
Henceforth, it is required for the sensor phase-shifted signals to also be modulated before they are reflected back.
However, in order to add the modulation block, it is required that the sensor also passes the signals through instead of just reflecting it back, as discussed in the previous subsection. We will now show how \name sensor design actually achieves thru-mode phase modulation which allows it to integrate with modulation blocks.

To show how \name works in thru mode, we move the sensor in the middle of the PCB simulations (Fig. \ref{fig:sensor_vna_res}) as compared to towards the end as shown in previous subsection. This allows us to define 2 lumped ports, one of each end of the PCB, and by observing S12 phase and magnitude we can verify if the sensor can work in a thru mode. For this simulation we obtain the S12 phase changes and observe that the phase changes are about half the magnitude we had before, that is 10$^{o}$ for 0-6 N forces as compared to 20$^{o}$ before. Now, when we keep the other port as reflective and estimate the S11 phase, we get almost the same phase shifts as before (around 20$^{o}$).

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{results/init_figs/thruPCB_sims.pdf}
    \caption{Phase doubling effect due to two sided travel via sensor: simulations}
    \label{fig:sensor_vna_res}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/init_figs/sens_mod_fin.pdf}
    \caption{Placement of sensor modulation block}
    \label{fig:sens_modulation_fin}
\end{figure}

Hence, intuitively what happens is that when a signal $s(t)$ travel through the sensor, it first gets a certain value of phase shift and the sensor passes the signal through $s(t)e^{j\phi(F_{\text{mag}})/2}$. Then, when the signals get modulated $s(t)e^{j\phi(F_{\text{mag}})/2}m(t)$, reflect and pass through the sensor again, the total phase shift doubles up $s(t)e^{j\phi(F_{\text{mag}})}m(t)$ and reaches back to the reflective levels as described in Eqn \eqref{eq:phase}. 
This is visually illustrated in Fig. \ref{fig:sens_modulation_fin}
Thus, the reflected signal has both the modulation component, as well as a phase shift. 
The wireless reader can use the modulation to isolate the sensor reflections from the environmental reflections and then estimate these phase shifts from the isolated signal.
This can be done by using any standardized demodulation block to isolate the sensor signals and then from the estimated channel these phase shifts can be computed.
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{implementation/impl.pdf}
    \caption{Interfacing the sensor with RFID tags: 
    % (a) Sensor prototype with two tungsten wire filaments compared to a dime coin 
    (a) Using a tweezer to peel away the RFID IC from the antenna (b) Placing the sensor tungsten wires below the conductive pads for the IC and (c) Final sensor + RFID prototype}
    \label{fig:my_label}
\end{figure*}

\subsection{Putting it all together: \name sensor with COTS RFIDs}
\begin{itemize}
    \item \textbf{Here we just describe the end-to-end process and how the phases are cleaned and processed}
\end{itemize}
In order to demonstrate wireless, batteryless force sensing we integrate our designed sensor prototype with RFIDs.
RFID technology has matured over the past decade and today there are commercial ICs available ~\cite{} which integrate a full-fledged energy harvestor and modulator logic. We can integrate the sensor with these RFID ICs, as well as COTS available RFIDs via certain fabrication techniques discussed in Section \ref{sec:implementation}. However, in effect, from a design point of view, the sensor is interfaced in parallel to the RFID modulation block, as shown in Fig. \ref{fig:sens_modulation_fin}.
% There has been one past challenge paper \cite{} which motivates integrating temperature, photo and binary touch/no-touch sensors based majorly on change in resistance with RFIDs.
% The major issue with the paper was that integrating resistive sensors with RFIDs lead to reduced range.



Since \name's capacitative force sensor has negligible resistive impedance, it only effects the phases of the signals passing through, and thus the input to the energy harvestor unit is the same magnitude signal as it would have been without the sensor. Hence, \name's method of integration does not adversely affect the RFID reading ranges.



To tie up \name's design, the only component left to describe is the wireless reader.
As explained towards end of previous subsection, \name sensor can use any COTS RFID reader which performs RFID channel estimates.
The COTS RFID reader can identify the signals coming from the sensor via figuring out the EPC id number of the RFID IC integrated with sensor.
Then, the RFID reader can observe the channel estimates of this particular tag and calculate sensor phase jumps to estimate applied forces. 

In order to estimate these phase jumps with COTS readers a challenge is the hopping nature of these COTS readers. As per FCC guidelines the readers need to change their frequencies after every 200 milliseconds to avoid interference with other readers in the environment. Most of the COTS readers introduce a random phase offset due to hopping which could show up in the phase calculations.
However, \name's sensing is robust to these random phase offsets as the phase change introduced by the force appears across each channel as a differential phase jump (Fig. ). Hence, \name calculates the phase jumps at each of the RFID hopping frequencies and then averages them to obtain a very clean phase jump measurement (to about 1$^o$ precision) which can then be used to compute the applied forces from the batteryless miniaturized sensor.
% However, \name operates on self-differential phase instead of absolute phase, that is, to determine the force applied \name estimates the only the change in phase across the , which automatically removes any of these fixed offsets.

% Prior work ~\cite{} puts forward a challenge in achieving the same: it shows how errors in RFID sensing can be substantial. The metrics considered there were phase, RSSI and DMRT: and it was considred how stable these quantities are. However, they didnt tuen off hopping: doing this with hopping could be a challenge. Dont go in this much detail: just tell its a challenge and they didnt consider time differential phase, and WiForce another past work basically relied on OFDM transforms which are not avaialble to RFID?

% in augmenting sensors to RFIDs ended up using series resistors which sense quantities by sensing relative drop in RSSIs of co-located tags. However, this requires presence of a second tag to take reference tag and further series networks are not generalizable (How to design something which notches/whatever DMRS did was to basically terse around RSSI problems via reference tag). But 

% \subsubsection{Single frequency based search}

% \subsubsection{Hopping based algorithm}



% \subsection{How \name integrates seamlessly with any wireless technology}

% Finally, here we can write two things:

% \begin{itemize}
%   \item Reading via switch based OFDM backscatter like we did in WiForce: however counter doppler now
%   \item RFID based stuff which we are doing now
% \end{itemize}


==> intros/intro_OG.tex <==
% !TEX root = paper.tex

\section{Introduction}

Over the past decade Microelectromechanical (MEMS) sensors have narrowed down the gap between the physical world and the digital world. 
A cornerstone of such MEMS sensing technologies are force sensors, which digitize the contact force acting upon them.
There has been a huge adoptation of force sensors in technologies like smartphones, smartwatches, airpods etc, which have batteries and processing power to interface these sensors. 
% The reason being that contact force is a fundamental quantity in action across all the walks of life, with objects
However today's force sensors can not be used for applications with resource constraints; where we can not assume a wired link or the luxury of putting a battery.

For example, today as robot technologies evolve, we need force sensors to be interfaced in multiple difficult to mount positions across the robot. 
We can not afford to have a bunch of wires running across to interface with these multiple force sensors, neither can we assume a small battery at each sensor so that it transmits the force readings wirelessly. Similar examples are that of surgical equipments safety and orthopaedic implants.
When a surgeon operates in-vivo on a body organ via the surgical equipment, excessive force applied on the organ by the equipment can damage it's tissues. Thus it is important for safe surgeries in the future to incorporate force sensors. 
Similar to this, the health of orthopaedic implants (for example knee implant) depends on how well it is able to sustain the contact forces between the joints. 
The implants can greatly benefit from a force sensor, which would be able to characterize the proper working and longevity of the same.
With today's force sensors, which demand wires and battery, none of these applications are possible.

% sensor just like a sticker
In order to achieve these applications, a key requirement is to design batteryless and wireless methods to read force sensors.
Further, an added requirement is of miniaturization, since, most of these applications of batteryless wireless sensors are at resource constraint places which are hard to mount, or are in-vivo surgical/orthopedic applications.
Hence, the sensor should be miniaturized enough so that it can fit to the in-vivo applications as well as get integrated at difficult to mount positions on the robot.

In this paper we present \name, the first force sensor prototype which meets all these three requirements. The key insight \name has to create this sensor is direct interfacing of the most widely miniaturized capacitative force sensor designs to RF backscatter interrogation. This direct interfacing allows \name to capitalize on years of research on both, miniaturized MEMS capacitative wired force sensors, as well batteryless wireless backscatter systems.
The past work in wireless force sensing \cite{} have designed a macro-scale sensor (sensor size: 80mm $\times$ 10mm $\times$ 5mm, final system with antennas+RF switches not integrated) and specialized electronics for backscatter modulation, which require significant research ahead in order to make it miniaturized and commercially viable in form of an IC. \name sensor (4mm $\times$ 2mm $\times$ 0.3mm, with small RFID antenna 16mm $\times$ 10mm $\times$ 0.5mm) avoids reinventing the wheel by using already proven sensor designs and COTS backscatter ICs.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_fig_1.pdf}
    \caption{\name sensor form factor and applications}
    \label{fig:intro_fig1}
\end{figure}

Hence, by directly interfacing the research efforts from both sensing and backscatter fields, \name takes a big leap in wireless force sensing by demonstrating a practically viable batteryless wireless sensor. The first component of \name is the capacitative force sensor design. Here, we design an approximation of a simple parallel plate capacitor filled with soft polymer dielectric. As the force is applied on the capacitor, the plates get closer to each other by compressing the soft polymer, which increases the capacitance in effect. This method of force to capacitance transduction is a common theme in MEMS sensor past works \cite{} as these capacitative designs are much easier to miniaturize as compared to other available force sensor designs like resistive sensors and load cells\cite{}. 

However, capacitative sensors can not be read directly via ADCs available in low-power microcontrollers, and require a dedicated CDC block (Capacitance to digital converters) which is absent in the batteryless backscatter communication platforms today.
Some advanced platforms do allow for an ADC to read sensor values, which can be used for resistive sensing as resistive sensors lead to voltage changes which can be read easily via ADCs. However, resisitve sensors can not be miniaturized easily and thus with a naive method of digitizing the sensor values via ADC and transmitting these digital bits, it is not possible to create a miniaturized force sensor.

This leads us to the second component of \name sensor design, where we make a key observation that when we integrate these force sensitive capacitors directly to RF frequencies, the change in capacitance leads to a  change in signal phase. 
% In order to get these phase shifts the capacitance has to be connected in p
The reason for this phase shift is that capacitative sensors show almost purely imaginary impedance and negligible real component.
Hence, when the signals pass through this imaginary impedance, the signal magnitude doesn't change, but they get phase shifted with the value of phase shift depending on the value of capacitance.
This intuition of how capacitors when operated directly at RF frequencies would give phase changes allows for direct 
RF interrogation of capacitance values which can then be used to determine the applied force.

Now with this model of capacitance mapping to phase shifts, we describe the final design component of \name. 
Since the capacitative sensors pass through the signals after applying a certain phase shift, we can feed these signals to a standard backscatter block which would modulate the phase shifted signals and reflect them back.
The added modulation would allow a remotely located wireless reader to isolate the sensor phase shifted signals from the myriad of environmental reflections. The modulation would require certain amount of power, however these power requirements can be met via RF energy harvesting.
Since the capacitative sensors just phase shift and do not affect the signal magnitude, the energy harvester block is not affected by the sensor and the modulation ranges remain consistent.
Hence, the capacitative sensor design can simply piggyback on top of any existing backscatter platform by creating phase changes as a function of applied forces, without affecting their reading ranges.

Thus, we build an end-to-end system around the capacitative sensor, we integrate it with RFIDs. Since there is a unique RFID connected to a sensor, we can identify the sensor signals by noticing the EPC ID (unique id given to each RFID) reported by the RFID readers.
Then by noticing the phase shifts in the channel associated with these EPC IDs we can estimate the applied force on the sensor. This also allows for multiple sensors to be read simultaneously, by piggybacking on top of well-developed RFID MAC layer.

We fabricate the capacitative sensors and integrate them with RF PCBs to experimentally evaluate \name's concept of force sensitive capacitor which leads to RF phase changes. 
The sensor by itself is 100x lower area form factor as compared to past work ~\cite{} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained match our intuition about capacitance to phase changes via FEM multiphysics simulations in Comsol. Finally, we integrate the sensors to RFIDs and read the phase changes wirelessly, and achieve a force error of xx N. We also show that the wireless reading of sensor is robust to propagation under tissue phantom. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model.


% Via the means of MEMS sensors, today our digital interfaces are very capable of sensing for example, temperature, humidity, touch vs no-touch among various other physical world parameters. The driving force behind the popularity of such sensors, was the engineering innovations which led to miniaturized sensor designs, allowing easy integration with technologies like smartphones/smart watches.

% batteryless sensing and possible applications



==> intros/introv2_old.tex <==
% !TEX root = paper.tex

\section{Introduction}

Over the past decade Microelectromechanical (MEMS) sensors have narrowed down the gap between the physical world and the digital world. 
A cornerstone of such MEMS sensing technologies are force sensors, which digitize the contact force acting upon them.
There has been a huge adoptation of force sensors in technologies like smartphones, smartwatches, airpods etc, which have batteries and processing power to interface these sensors. 
% The reason being that contact force is a fundamental quantity in action across all the walks of life, with objects
However today's force sensors can not be used for applications which are energy and space constraint. 
In other words, we can not use today's force sensors at places where we do not have the luxuries of putting batteries, or neither the real estate required to carry wires to each sensor for force feedback. 
% which have limited space available to mount the sensors and niether a luxury to carry wires
% in form of limited space to mount the sensors, or 

An application area where we can clearly see the energy+space constraint are the various medical use-cases of force sensors. 
Here the sensor has to be small enough to operate inside the body (in-vivo), and transmit the sensor wirelessly through the tissue layers as we can not carry wires inside the body, that too in a battery-free manner since batteries could post a big contamnination risk when used in-vivo.
Some examples of in-vivo applications include augmenting surgical tools with battery-free force sensors for safer surgeries by providing the surgeon with the required contact force feedback, and orthopaedic implant health monitoring by sensing the forces which the implant handles as various parts of the joint are moved to verify the implant's capability to sustain these joint contact forces.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_fig_1.pdf}
    \caption{\name sensor form factor and applications}
    \label{fig:intro_fig1}
\end{figure}


Another application area with these energy+space constraint is the field of soft robotics.
Here, the robots utilize unconventionally flexible designs to make the robot take various shapes and form factors, in order to better navigate tight constraints.
% Soft robots find various applications, like helping with disaster management rescue, automation of surgeries etc.
In order to make this vision of soft robotics possible, it is highly imperative to sense the forces applied by the robot on the environment, as it goes from one shape configuration to other.
Doing so would require placing multiple force sensors throughout the length of the soft robot,
which are small enough to confrim well to the various changing shapes and not requiring a battery/wired power link per sensor which would hinder the flexibility of the soft robot.


% % sensor just like a sticker
% In order to achieve these applications, a key requirement is to design batteryless and wireless methods to read force sensors.
% Further, an added requirement is of miniaturization, since, most of these applications of batteryless wireless sensors are at resource constraint places which are hard to mount, or are in-vivo surgical/orthopedic applications.
% Hence, the sensor should be miniaturized enough so that it can fit to the in-vivo applications as well as get integrated at difficult to mount positions on the robot.

In this paper we present \name (Fig. \ref{fig:intro_fig1}), the first force sensor prototype which meets the space and energy constraints simultaneously. 
The key idea behind \name is the confluence of the widely-adopted and mechanically proven miniaturized wired capacitative force sensor design and with the most low-power, energy efficient wireless backscatter communications.
% The key insight \name has to create this sensor is direct interfacing of the most widely miniaturized capacitative force sensor designs to RF backscatter interrogation. 
Hence, \name's capacitative backscatter approach  capitalizes on years of research on both, miniaturized MEMS force sensors, as well batteryless wireless systems to deliver a miniaturized batteryless force sensor.
The past work in wireless force sensing \cite{} has designed a 80mm $\times$ 10mm $\times$ 5mm sensor which doesn't have an end-to-end integrated system since the sensor requires  specialized electronics for the backscatter modulation, which further require significant research ahead in order to make it miniaturized and commercially viable in form of an IC. \name sensor measures 4mm $\times$ 2mm $\times$ 0.3mm, $>$1000x smaller in terms of volume, and is integrated with commercially available backscatter ICs today, hence avoiding reinventing the wheel by both, using already proven capacitative sensor designs and COTS backscatter ICs.

Hence, by directly interfacing the research efforts from both sensing and backscatter fields, \name takes a big leap in wireless force sensing by demonstrating a practically viable mm-scale batteryless wireless sensor. The first component of \name is the capacitative force sensor design. Here, we design an approximation of a simple parallel plate capacitor filled with soft polymer dielectric. As the force is applied on the capacitor, the plates get closer to each other by compressing the soft polymer, which increases the capacitance in effect. This method of force to capacitance transduction is a common theme in MEMS sensor past works \cite{} as these capacitative designs are much easier to miniaturize as compared to other available force sensor designs like resistive sensors and load cells\cite{}. 

However, capacitative sensors can not be read directly via ADCs available in low-power microcontrollers, and require a dedicated CDC block (Capacitance to digital converters) which is absent in the batteryless backscatter communication platforms today.
% Some advanced platforms do allow for an ADC to read sensor values, which can be used for resistive sensing as resistive sensors lead to voltage changes which can be read easily via ADCs. However, resisitve sensors can not be miniaturized easily and thus with a naive method of digitizing the sensor values via ADC and transmitting these digital bits, it is not possible to create a miniaturized force sensor.
This leads us to the second component of \name sensor design, where we make a key observation that when we integrate these force sensitive capacitors directly to RF frequencies, the change in capacitance leads to a  change in signal phase. 
% In order to get these phase shifts the capacitance has to be connected in p
The reason for this phase shift is that capacitative sensors show almost purely imaginary impedance and negligible real component.
Hence, when the signals pass through this imaginary impedance, the signal magnitude doesn't change, but they get phase shifted with the value of phase shift depending on the value of capacitance.
This intuition of how capacitors when operated directly at RF frequencies would give phase changes allows for direct 
RF interrogation of capacitance values which can then be used to determine the applied force, without requiring a dedicated CDC block in existing backscatter systems.

Now with this model of capacitance mapping to phase shifts, we describe the final design component of \name. 
Since the capacitative sensors pass through the signals after applying a certain phase shift, we can feed these signals to a standard backscatter block which would modulate the phase shifted signals and reflect them back.
The added modulation would allow a remotely located wireless reader to isolate the sensor phase shifted signals from the myriad of environmental reflections. The modulation would require certain amount of power, however these power requirements can be met via RF energy harvesting.
Since the capacitative sensors just phase shift and do not affect the signal magnitude, the energy harvester block is not affected by the sensor and the modulation ranges remain consistent.
Hence, the capacitative sensor design can simply piggyback on top of any existing backscatter platform by creating phase changes as a function of applied forces, without affecting their reading ranges.

Thus, we build an end-to-end system around the capacitative sensor, we integrate it with RFIDs. Since there is a unique RFID connected to a sensor, we can identify the sensor signals by noticing the EPC ID (unique id given to each RFID) reported by the RFID readers.
Then by noticing the phase shifts in the channel associated with these EPC IDs we can estimate the applied force on the sensor. This also allows for multiple sensors to be read simultaneously, by piggybacking on top of well-developed RFID MAC layer.

We fabricate the capacitative sensors and integrate them with RF PCBs to experimentally evaluate \name's concept of force sensitive capacitor which leads to RF phase changes. 
The sensor by itself is 100x lower area form factor as compared to past work ~\cite{} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained match our intuition about capacitance to phase changes via FEM multiphysics simulations in Comsol. Finally, we integrate the sensors to RFIDs and read the phase changes wirelessly, and achieve a force error of xx N. We also show that the wireless reading of sensor is robust to propagation under tissue phantom. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model.


% Via the means of MEMS sensors, today our digital interfaces are very capable of sensing for example, temperature, humidity, touch vs no-touch among various other physical world parameters. The driving force behind the popularity of such sensors, was the engineering innovations which led to miniaturized sensor designs, allowing easy integration with technologies like smartphones/smart watches.

% batteryless sensing and possible applications



==> intros/introv3.tex <==
% !TEX root = paper.tex

\section{Introduction}

Over the past decade Microelectromechanical (MEMS) sensors have narrowed down the gap between the physical world and the digital world\cite{}. 
A cornerstone of such MEMS sensing technologies are force sensors, which digitize the contact force acting upon them.
There has been a huge adoptation of force sensors in technologies like smartphones, smartwatches, airpods \cite{} which have batteries and processing power to interface these sensors. 
% The reason being that contact force is a fundamental quantity in action across all the walks of life, with objects
However today's force sensors can not be used for applications which are energy and space constraint. 
In other words, we can not use today's force sensors at places where we do not have the luxuries of putting batteries, or neither the real estate required to carry wires to each sensor for force feedback. 
% which have limited space available to mount the sensors and niether a luxury to carry wires
% in form of limited space to mount the sensors, or 

An application area where we can clearly see the energy+space constraint are the various medical use-cases of force sensors. 
Here the sensor has to be small enough to operate inside the body (in-vivo), and transmit the sensor wirelessly through the tissue layers as we can not carry wires inside the body\cite{}, that too in a battery-free manner since batteries could post a big contamination risk when used in-vivo\cite{}.
Some examples of in-vivo applications include augmenting surgical tools with battery-free force sensors for safer surgeries by providing the surgeon with the required contact force feedback\cite{}, and orthopaedic implant health monitoring by sensing the forces which the implant handles as various parts of the joint are moved to verify the implant's capability to sustain these joint contact forces\cite{}.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_fig_1.pdf}
    \caption{\name sensor form factor and applications}
    \label{fig:intro_fig1}
\end{figure}


Another application area with these energy+space constraint is the field of soft robotics\cite{}.
Here, the robots utilize unconventionally flexible designs to make the robot take various shapes and form factors, in order to better navigate tight constraints.
% Soft robots find various applications, like helping with disaster management rescue, automation of surgeries etc.
In order to make this vision of soft robotics possible, it is highly imperative to sense the forces applied by the robot on the environment, as it goes from one shape configuration to other\cite{}.
Doing so would require placing multiple force sensors throughout the length of the soft robot,
which are small enough to confrim well to the various changing shapes and not requiring a battery/wired power link per sensor which would hinder the flexibility of the soft robot.


% % sensor just like a sticker
% In order to achieve these applications, a key requirement is to design batteryless and wireless methods to read force sensors.
% Further, an added requirement is of miniaturization, since, most of these applications of batteryless wireless sensors are at resource constraint places which are hard to mount, or are in-vivo surgical/orthopedic applications.
% Hence, the sensor should be miniaturized enough so that it can fit to the in-vivo applications as well as get integrated at difficult to mount positions on the robot.

In this paper we present \name (Fig. \ref{fig:intro_fig1}), the first force sensor prototype which meets the space and energy constraints simultaneously. 
Capacitative force sensors are the most widely miniaturized, as well as mechanically robust force sensors\cite{} and by themselves solve for the space constraints.
On the other hand, wireless backscatter systems like RFIDs solve for the energy constraints by eliminating battery requirements and instead using RF energy harvesting \cite{}.
\name piggybacks on years of research on both
miniaturized MEMS force sensors, as well backscatter wireless systems, to create a batteryless miniaturized sensor.


Thus, the natural question is how does \name bring these two vastly different research fields together. The first step in the process is to create a force sensitive capacitative sensor which works well at RF frequencies.
That is, the sensor shows sufficient capacitance changes due to applied forces, and not create non-idealities like signal losses/resonant frequency changes when used at RF frequencies.
For this, we design a parallel plate capacitor which essentially has a soft polymer layer in middle acting as dielectric sandwiched between two copper plates.
As force on the copper plates increase, the soft layer deforms and the two plates come closer to each other which increases the capacitance.
\name designs this capacitative sensor via help of Comsol multiphysics FEM simulations (by solving both structural mechanics as well as maxwell equations) to confirm the goodness of the designed sensor's capacitative effect at high RF frequencies.

Now, a naive way to
interface this capacitative sensor to backscatter systems is to incorporate a CDC (Capacitance to Digital Converters) and communicate the digitized values via digital backscatter communications.
However, the CDC block is a specialized entity and extremely power hungry, and hence not present in any existing backscatter systems.
Instead of doing a ground-up redesign of backscatter systems to incorporate CDCs, \name makes a key observation that change in capacitance caused by force leads to measureable phase shifts. The reason for this phase shift is that capacitors at RF frequencies show purely imaginary impedance and negligible real component.
Hence, when the signals pass through this imaginary impedance, the signal magnitude doesn't change, but they get phase shifted with the value of phase shift depending on the value of capacitance (and hence force).
This intuition of how capacitors when operated directly at RF frequencies would give phase changes allows for direct 
RF interrogation of capacitance to determine the applied force, without requiring redesign of existing backscatter systems.

However, with the capacitative phase shifts a natural question is how can we measure these phase shifts wirelessly and with the required accuracy. 
Since the capacitative sensors pass through the signals after applying a certain phase shift, we can feed these signals to a standard backscatter block which would modulate the phase shifted signals and reflect them back.
The added modulation would allow a remotely located wireless reader to isolate the sensor phase shifted signals from the myriad of environmental reflections. The modulation would require certain amount of power, however these power requirements can be met via RF energy harvesting.
Since the capacitative sensors just phase shift and do not affect the signal magnitude, the energy harvester block is not affected by the sensor and the modulation ranges remain consistent.
Hence, the capacitative sensor design can simply piggyback on top of any existing backscatter platform by creating phase changes as a function of applied forces, without affecting their reading ranges.

Thus, we build an end-to-end system around the capacitative sensor, we integrate it with existing COTS RFIDs. 
Today the existing COTS RFIDs integrate a small flexible antenna and an IC which performs energy harvesting and low-power backscatter modulation (Fig. 1).
By interfacing the capacitative sensor with these RFIDs, we automatically borrow these small flexible form factors as well as batteryless operation of RFIDs.
Since there is a unique RFID connected to a sensor, we can identify the sensor signals by noticing the EPC ID (unique id given to each RFID) reported by the RFID readers.
Then by noticing the phase shifts in the channel associated with these EPC IDs we can estimate the applied force on the sensor. This also allows for multiple sensors to be read simultaneously, by piggybacking on top of well-developed RFID MAC layer.

Hence, to summarize, we fabricate the capacitative sensors which work successfully at RF frequencies and integrate them with RF PCBs to experimentally evaluate \name's concept of force sensitive capacitor which leads to RF phase changes. 
The sensor by itself is 1000x lower volume form factor as compared to recent past work ~\cite{} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained match our intuition about capacitance to phase changes via FEM multiphysics simulations in COMSOL. Finally, we integrate the sensors to RFIDs and read the phase changes wirelessly, and achieve a force error of xx N. We also show that the wireless reading of sensor is robust to propagation under tissue phantom. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model.


% Via the means of MEMS sensors, today our digital interfaces are very capable of sensing for example, temperature, humidity, touch vs no-touch among various other physical world parameters. The driving force behind the popularity of such sensors, was the engineering innovations which led to miniaturized sensor designs, allowing easy integration with technologies like smartphones/smart watches.

% batteryless sensing and possible applications



==> intros/introv4.tex <==
% !TEX root = paper.tex

\section{Introduction}

Every human interaction and/or robot actuation relies on applying or sensing the forces of that interaction, thus enabling force sensing has many applications. For example, in-vivo applications include augmenting surgical tools with battery-free force sensors for safer surgeries by providing the surgeon with the required contact force feedback\cite{}, and orthopaedic implant health monitoring by sensing the forces which the implant handles as various parts of the joint are moved to verify the implant's capability to sustain these joint contact forces\cite{}. 

Such applications require a specialized force sensor with new requirements. The sensor has to be small enough to operate inside the body (in-vivo), and transmit the sensor information wirelessly through the tissue layers as we can not carry wires inside the body\cite{}, that too in a battery-free manner since batteries could post a big contamination risk when used in-vivo\cite{}.
Furthermore, in the field of soft robotics\cite{}\footnote{Soft robots find various applications, like helping with disaster management rescue, automation of surgeries etc.}, the robots utilize unconventionally flexible designs to make the robot take various shapes and form factors, in order to better navigate tight constraints.
In order to make this vision of soft robotics possible, it is highly imperative to sense the forces applied by the robot from the environment, as it goes from one shape configuration to other\cite{}.
Doing so would require placing multiple force sensors throughout the length of the soft robot,
which are small enough to confirm well to the various changing shapes and not requiring a battery/wired power link per sensor which would hinder the flexibility of the soft robot. In summary, we need a wireless force sensor, which is flexible, space efficient and energy efficient or battery-free.


Over the past two decades, reserachers have designed micro-electro-mechanical sensors (MEMS) which digitize the contact force acting upon them. There has been a huge adoptation of force sensors in technologies like smartphones, smartwatches, airpods \cite{} which have batteries and processing power to interface these sensors. 
% The reason being that contact force is a fundamental quantity in action across all the walks of life, with objects
However these force sensors can not be used for applications which require wireless, flexible, energy-efficient and space constraint. 
In other words, we can not use today's force sensors at places where we do not have the luxuries of putting batteries, or neither the real estate required to carry wires to each sensor for force feedback. On the other hand, a recent work develops wireless force sensor for continnum robots, which develops a rather large sensor, which could have worked if it can measure multiple force interaction along its length. However, it cannot, furthermore, the design is neither flexible, nor batteryfree.  
% which have limited space available to mount the sensors and niether a luxury to carry wires
% in form of limited space to mount the sensors, or 



\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_fig_1.pdf}
    \caption{\name sensor form factor and applications}
    \label{fig:intro_fig1}
\end{figure}


% % sensor just like a sticker
% In order to achieve these applications, a key requirement is to design batteryless and wireless methods to read force sensors.
% Further, an added requirement is of miniaturization, since, most of these applications of batteryless wireless sensors are at resource constraint places which are hard to mount, or are in-vivo surgical/orthopedic applications.
% Hence, the sensor should be miniaturized enough so that it can fit to the in-vivo applications as well as get integrated at difficult to mount positions on the robot.

In this paper, therefore, we present \name (Fig. \ref{fig:intro_fig1}), the first flexible, wireless force sensor prototype which meets the space constraint (xx mm X yy mm) and battery free all in one. \name develops a novel capacitive flexible force sensor, which leverages capacitor phenomena but can induce the force applied to create change in the wireless channel, which then can be measured wirelessly by just observing the phase change. \name integrates the flexible force sensor with popularly and widely available RFID-tags, which then enables us to power the sensor wirelessly and read the force passively by just observing the wireless channel change, basically enabling jointly power and communication paradigm for the sensor. \name integrates its flexible capacitive force sensor in the path of reading RFID-tag, specifically it places sensor between the RFID-tag chip and flexible RFID-antenna, and form a flexible contraption as shown in Fig. xx. \name force sensor is read by interrogating the tag, and processing the wireless channel of tag to infer the force. \name sensor requires COTS RFID reader, with processing algorithms to read the sensor upto 5 meter range even inside the body. \name's system design is robust, as it conceptually leverages years of research on both miniaturized MEMS force sensors, as well backscatter wireless systems, to create a batteryless miniaturized sensor.

\name's first challenge lies in designing the flexible force sensors, that can induce wireless channel change. A natural way to develop such sensor is leverage existing capacitive force sensors, those are most widely miniaturized, as well as mechanically robust force sensors\cite{}. However, the traditional capacitive force sensor provide capacitance change in the order of xx with quality factor, which fundamentally cannot cause a wireless channel change at low-loss at RF frequencies.  


Thus, the natural question is how does \name bring these two vastly different research fields together. The first step in the process is to create a force sensitive capacitative sensor which works well at RF frequencies.

That is, the sensor shows sufficient capacitance changes due to applied forces, and not create non-idealities like signal losses/resonant frequency changes when used at RF frequencies.
For this, we design a parallel plate capacitor which essentially has a soft polymer layer in middle acting as dielectric sandwiched between two copper plates.
As force on the copper plates increase, the soft layer deforms and the two plates come closer to each other which increases the capacitance.
\name designs this capacitative sensor via help of Comsol multiphysics FEM simulations (by solving both structural mechanics as well as maxwell equations) to confirm the goodness of the designed sensor's capacitative effect at high RF frequencies.

Now, a naive way to
interface this capacitative sensor to backscatter systems is to incorporate a CDC (Capacitance to Digital Converters) and communicate the digitized values via digital backscatter communications.
However, the CDC block is a specialized entity and extremely power hungry, and hence not present in any existing backscatter systems.
Instead of doing a ground-up redesign of backscatter systems to incorporate CDCs, \name makes a key observation that change in capacitance caused by force leads to measureable phase shifts. The reason for this phase shift is that capacitors at RF frequencies show purely imaginary impedance and negligible real component.
Hence, when the signals pass through this imaginary impedance, the signal magnitude doesn't change, but they get phase shifted with the value of phase shift depending on the value of capacitance (and hence force).
This intuition of how capacitors when operated directly at RF frequencies would give phase changes allows for direct 
RF interrogation of capacitance to determine the applied force, without requiring redesign of existing backscatter systems.

However, with the capacitative phase shifts a natural question is how can we measure these phase shifts wirelessly and with the required accuracy. 
Since the capacitative sensors pass through the signals after applying a certain phase shift, we can feed these signals to a standard backscatter block which would modulate the phase shifted signals and reflect them back.
The added modulation would allow a remotely located wireless reader to isolate the sensor phase shifted signals from the myriad of environmental reflections. The modulation would require certain amount of power, however these power requirements can be met via RF energy harvesting.
Since the capacitative sensors just phase shift and do not affect the signal magnitude, the energy harvester block is not affected by the sensor and the modulation ranges remain consistent.
Hence, the capacitative sensor design can simply piggyback on top of any existing backscatter platform by creating phase changes as a function of applied forces, without affecting their reading ranges.

Thus, we build an end-to-end system around the capacitative sensor, we integrate it with existing COTS RFIDs. 
Today the existing COTS RFIDs integrate a small flexible antenna and an IC which performs energy harvesting and low-power backscatter modulation (Fig. 1).
By interfacing the capacitative sensor with these RFIDs, we automatically borrow these small flexible form factors as well as batteryless operation of RFIDs.
Since there is a unique RFID connected to a sensor, we can identify the sensor signals by noticing the EPC ID (unique id given to each RFID) reported by the RFID readers.
Then by noticing the phase shifts in the channel associated with these EPC IDs we can estimate the applied force on the sensor. This also allows for multiple sensors to be read simultaneously, by piggybacking on top of well-developed RFID MAC layer.

Hence, to summarize, we fabricate the capacitative sensors which work successfully at RF frequencies and integrate them with RF PCBs to experimentally evaluate \name's concept of force sensitive capacitor which leads to RF phase changes. 
The sensor by itself is 1000x lower volume form factor as compared to recent past work ~\cite{} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained match our intuition about capacitance to phase changes via FEM multiphysics simulations in COMSOL. Finally, we integrate the sensors to RFIDs and read the phase changes wirelessly, and achieve a force error of xx N. We also show that the wireless reading of sensor is robust to propagation under tissue phantom. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model.


% Via the means of MEMS sensors, today our digital interfaces are very capable of sensing for example, temperature, humidity, touch vs no-touch among various other physical world parameters. The driving force behind the popularity of such sensors, was the engineering innovations which led to miniaturized sensor designs, allowing easy integration with technologies like smartphones/smart watches.

% batteryless sensing and possible applications



==> intros/introv5.tex <==
% !TEX root = paper.tex

\section{Introduction}
\begin{itemize}[leftmargin=0pt]
    \item \textbf{All objects/human interactions happen due to contact force, sensing forces ubiquitously can capture and quantify/digitize a lot of information about environment}
    \item \textbf{However, this requires a force sensor which can be stuck around without disturbing the environment in the first place; it should confirm well to uneven surfaces and not require wires}
    \item \textbf{Not only ubiquitous sensing, such sticker-like sensors will also enable new medical applications which also require similar batteryless sensing approaches}
    \item \textbf{We present \name which is the first such sensor to achieve these applications.. }
    \item \textbf{Our key insight is to design a <1mm thick miniaturized capacitive force sensor at 900 MHz RFID frequencies, where it acts akin to a force sensitive varactor}
    \item \textbf{The force sensitive varactor design creates changes in wireless channel by shifting signal phases due to application of force, which is utilized to read the sensor wirelessly}
    \item  \textbf{We simulate the sensor in a multiphysics simulator to confirm it's working at 900 MHz. 
    Further, we also show how sensor can be integrated with existing RFID backscatter systems to allow for wireless operation}
    \item \textbf{We also show how to have the sensor as a PCB component with a designed PCB pad for easy interfacing with antennas and ICs. We also show a small antenna designs to improve on the form factor}
    \item \textbf{Finally, we build algorithms to sense phase from RFID reader reliably to sense the force robustly}
    \item \textbf{Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications}
\end{itemize}
Every human interaction and/or robot actuation relies on applying or sensing the forces of that interaction, thus enabling force sensing has many applications. For example, in-vivo applications include augmenting surgical tools with battery-free force sensors for safer surgeries by providing the surgeon with the required contact force feedback\cite{}, and orthopaedic implant health monitoring by sensing the forces which the implant handles as various parts of the joint are moved to verify the implant's capability to sustain these joint contact forces\cite{}. 

Such applications require a specialized force sensor with new requirements. The sensor has to be small enough to operate inside the body (in-vivo), and transmit the sensor information wirelessly through the tissue layers as we can not carry wires inside the body\cite{}, that too in a battery-free manner since batteries could post a big contamination risk when used in-vivo\cite{}.
Furthermore, in the field of soft robotics\cite{}\footnote{Soft robots find various applications, like helping with disaster management rescue, automation of surgeries etc.}, the robots utilize unconventionally flexible designs to make the robot take various shapes and form factors, in order to better navigate tight constraints.
In order to make this vision of soft robotics possible, it is highly imperative to sense the forces applied by the robot from the environment, as it goes from one shape configuration to other\cite{}.
Doing so would require placing multiple force sensors throughout the length of the soft robot,
which are small enough to confirm well to the various changing shapes and not requiring a battery/wired power link per sensor which would hinder the flexibility of the soft robot. In summary, we need a wireless force sensor, which is flexible, space efficient and energy efficient or battery-free.


Over the past two decades, reserachers have designed micro-electro-mechanical sensors (MEMS) which digitize the contact force acting upon them. There has been a huge adoptation of force sensors in technologies like smartphones, smartwatches, airpods \cite{} which have batteries and processing power to interface these sensors. 
% The reason being that contact force is a fundamental quantity in action across all the walks of life, with objects
However these force sensors can not be used for applications which require wireless, flexible, energy-efficient and space constraint. 
In other words, we can not use today's force sensors at places where we do not have the luxuries of putting batteries, or neither the real estate required to carry wires to each sensor for force feedback. On the other hand, a recent work develops wireless force sensor for continnum robots, which develops a rather large sensor, which could have worked if it can measure multiple force interaction along its length. However, it cannot, furthermore, the design is neither flexible, nor batteryfree.  
% which have limited space available to mount the sensors and niether a luxury to carry wires
% in form of limited space to mount the sensors, or 



\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_fig_1.pdf}
    \caption{\name sensor form factor and applications}
    \label{fig:intro_fig1}
\end{figure}


% % sensor just like a sticker
% In order to achieve these applications, a key requirement is to design batteryless and wireless methods to read force sensors.
% Further, an added requirement is of miniaturization, since, most of these applications of batteryless wireless sensors are at resource constraint places which are hard to mount, or are in-vivo surgical/orthopedic applications.
% Hence, the sensor should be miniaturized enough so that it can fit to the in-vivo applications as well as get integrated at difficult to mount positions on the robot.

In this paper, therefore, we present \name (Fig. \ref{fig:intro_fig1}), the first flexible, wireless force sensor prototype which meets the space constraint (xx mm X yy mm) and battery free all in one. \name develops a novel capacitive flexible force sensor, which leverages capacitor phenomena but can induce the force applied to create change in the wireless channel, which then can be measured wirelessly by just observing the phase change. \name integrates the flexible force sensor with popularly and widely available RFID-tags, which then enables us to power the sensor wirelessly and read the force passively by just observing the wireless channel change, basically enabling jointly power and communication paradigm for the sensor. \name integrates its flexible capacitive force sensor in the path of reading RFID-tag, specifically it places sensor between the RFID-tag chip and flexible RFID-antenna, and form a flexible contraption as shown in Fig. xx. \name force sensor is read by interrogating the tag, and processing the wireless channel of tag to infer the force. \name sensor requires COTS RFID reader, with processing algorithms to read the sensor upto 5 meter range even inside the body. \name's system design is robust, as it conceptually leverages years of research on both miniaturized MEMS force sensors, as well backscatter wireless systems, to create a batteryless miniaturized sensor.

\name's first challenge lies in designing the flexible force sensors, that can induce wireless channel change. A natural way to develop such sensor is leverage existing capacitive force sensors, those are most widely miniaturized, as well as mechanically robust force sensors\cite{}. However, the traditional capacitive force sensor provide capacitance change in the order of xx with quality factor, which fundamentally cannot cause a wireless channel change at low-loss at RF frequencies.  


Thus, the natural question is how does \name bring these two vastly different research fields together. The first step in the process is to create a force sensitive capacitative sensor which works well at RF frequencies.

That is, the sensor shows sufficient capacitance changes due to applied forces, and not create non-idealities like signal losses/resonant frequency changes when used at RF frequencies.
For this, we design a parallel plate capacitor which essentially has a soft polymer layer in middle acting as dielectric sandwiched between two copper plates.
As force on the copper plates increase, the soft layer deforms and the two plates come closer to each other which increases the capacitance.
\name designs this capacitative sensor via help of Comsol multiphysics FEM simulations (by solving both structural mechanics as well as maxwell equations) to confirm the goodness of the designed sensor's capacitative effect at high RF frequencies.

Now, a naive way to
interface this capacitative sensor to backscatter systems is to incorporate a CDC (Capacitance to Digital Converters) and communicate the digitized values via digital backscatter communications.
However, the CDC block is a specialized entity and extremely power hungry, and hence not present in any existing backscatter systems.
Instead of doing a ground-up redesign of backscatter systems to incorporate CDCs, \name makes a key observation that change in capacitance caused by force leads to measureable phase shifts. The reason for this phase shift is that capacitors at RF frequencies show purely imaginary impedance and negligible real component.
Hence, when the signals pass through this imaginary impedance, the signal magnitude doesn't change, but they get phase shifted with the value of phase shift depending on the value of capacitance (and hence force).
This intuition of how capacitors when operated directly at RF frequencies would give phase changes allows for direct 
RF interrogation of capacitance to determine the applied force, without requiring redesign of existing backscatter systems.

However, with the capacitative phase shifts a natural question is how can we measure these phase shifts wirelessly and with the required accuracy. 
Since the capacitative sensors pass through the signals after applying a certain phase shift, we can feed these signals to a standard backscatter block which would modulate the phase shifted signals and reflect them back.
The added modulation would allow a remotely located wireless reader to isolate the sensor phase shifted signals from the myriad of environmental reflections. The modulation would require certain amount of power, however these power requirements can be met via RF energy harvesting.
Since the capacitative sensors just phase shift and do not affect the signal magnitude, the energy harvester block is not affected by the sensor and the modulation ranges remain consistent.
Hence, the capacitative sensor design can simply piggyback on top of any existing backscatter platform by creating phase changes as a function of applied forces, without affecting their reading ranges.

Thus, we build an end-to-end system around the capacitative sensor, we integrate it with existing COTS RFIDs. 
Today the existing COTS RFIDs integrate a small flexible antenna and an IC which performs energy harvesting and low-power backscatter modulation (Fig. 1).
By interfacing the capacitative sensor with these RFIDs, we automatically borrow these small flexible form factors as well as batteryless operation of RFIDs.
Since there is a unique RFID connected to a sensor, we can identify the sensor signals by noticing the EPC ID (unique id given to each RFID) reported by the RFID readers.
Then by noticing the phase shifts in the channel associated with these EPC IDs we can estimate the applied force on the sensor. This also allows for multiple sensors to be read simultaneously, by piggybacking on top of well-developed RFID MAC layer.

Hence, to summarize, we fabricate the capacitative sensors which work successfully at RF frequencies and integrate them with RF PCBs to experimentally evaluate \name's concept of force sensitive capacitor which leads to RF phase changes. 
The sensor by itself is 1000x lower volume form factor as compared to recent past work ~\cite{} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained match our intuition about capacitance to phase changes via FEM multiphysics simulations in COMSOL. Finally, we integrate the sensors to RFIDs and read the phase changes wirelessly, and achieve a force error of xx N. We also show that the wireless reading of sensor is robust to propagation under tissue phantom. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model.


% Via the means of MEMS sensors, today our digital interfaces are very capable of sensing for example, temperature, humidity, touch vs no-touch among various other physical world parameters. The driving force behind the popularity of such sensors, was the engineering innovations which led to miniaturized sensor designs, allowing easy integration with technologies like smartphones/smart watches.

% batteryless sensing and possible applications



==> intros/introv6.tex <==
% !TEX root = paper.tex
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{intros/introv6_fig_1.pdf}
    \caption{(a) Shows the 2 versions of \name (b) demonstrates the flexibility of the sensors (c) shows how \name can be stuck on bottom of packages to measure the weight of contents inside for integrity checks (d) shows how \name can be used for in-vivo implant force sensing and (e) shows a possible integration of \name sensor with tendon driven robots}
    \label{fig:intro_fig}
\end{figure}
\section{Introduction}
% \begin{itemize}[leftmargin=0pt]
%     \item \textbf{All objects/human interactions happen due to contact force, sensing forces ubiquitously can capture and quantify/digitize a lot of information about environment}
%     \item \textbf{However, this requires a force sensor which can be stuck around without disturbing the environment in the first place; it should confirm well to uneven surfaces and not require wires}
%     \item \textbf{Not only ubiquitous sensing, such sticker-like sensors will also enable new medical applications which also require similar batteryless sensing approaches}
%     \item \textbf{We present \name which is the first such sensor to achieve these applications.. }
%     \item \textbf{Our key insight is to design a <1mm thick miniaturized capacitive force sensor at 900 MHz RFID frequencies, where it acts akin to a force sensitive varactor}
%     \item \textbf{The force sensitive varactor design creates changes in wireless channel by shifting signal phases due to application of force, which is utilized to read the sensor wirelessly}
%     \item  \textbf{We simulate the sensor in a multiphysics simulator to confirm it's working at 900 MHz. 
%     Further, we also show how sensor can be integrated with existing RFID backscatter systems to allow for wireless operation}
%     \item \textbf{We also show how to have the sensor as a PCB component with a designed PCB pad for easy interfacing with antennas and ICs. We also show a small antenna designs to improve on the form factor}
%     \item \textbf{Finally, we build algorithms to sense phase from RFID reader reliably to sense the force robustly}
%     \item \textbf{Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications}
% \end{itemize}

% Force ubiquiti
\noindent Force is an ubiquitous phenomenon in our daily environment, with any two objects in contact exerting forces onto each other.
In case of an object in contact with a table, there would be the objects weight (gravitational force) exerted onto the table.
Another example of two objects in contact could be our bone joints, which create movement by exerting the interaction forces on the other bones and ligaments in contact via the joint.
Force sensors can quantify these ubiquitous contact phenomenon, and bridge the gap between the digital world and the real environment.

% Any object would exert it's weight (gravitational force) onto it's support, and our range of daily activities involves various interaction forces between various bone joints and ligaments, among various other examples. 
% % However, a lack of ubiquitously available force sensors lead to these interactions not being recorded and quantified, creating a big gap between our digital world and the real environment.

Hence, force sensors enable myriad of applications, in diverse fields like warehouse scenarios, orthopaedic implants and robotics.
For example, we could sense the weight of packages in a warehouse setting, and then use it for integrity checks~\cite{}, since an empty or improperly packed package would apply a lower gravitational force. 
Similarly, an orthopaedic implant equipped with a force sensor could measure the contact forces between the knee joints as the patient recovers post-surgery to categorize the implant health and how well the body accepts the knee implant~\cite{}. 
Another application area is robotics, where these force sensors can be used to better control the robots, for example while gripping a sensitive objects the robotic manipulator needs to quantify the forces it is applying~\cite{}, and in surgical robots which have to be careful while interacting with body tissues so that they don't damage the tissues by applying excessive forces~\cite{}. 
% in field of surgical robots which navigate in tight in-vivo spaces where the robot can 

However, these applications pose numerous challenges, and hence are not mainstream today.
In order to ubiquitously sense weight in warehouse settings, requiring a full-fledged weighing scale below the packages to measure weight won't be practical, and hence we need to create force sensors which can be simply stuck to the bottom of the packages like a barcode and be read wirelessly to measure the weight of the contents.
Further, such sensors, if made miniaturized enough and flexible, can also confirm to the uneven shapes of orthopaedic implants and read the bone joint forces.
In addition to form-factor and flexibility requirements, such in-vivo applications would also require batteryless operation, since we can not have risk of contamination by carrying small coin cell batteries inside the body.
Further, such battery-free wireless force stickers can fulfill robotic applications which also require force sensors to be mount in unusual space constraint places. 
With today's force sensing technologies, most of them being wired, or requiring batteries, fabricating such force-sensitive stickers is impossible and hence these applications remain hypothetical and researched in laboratory settings only to show potential benefits of force sensing, hence force sensors aren't a ubiquitous part of our daily life.

In this paper, we present \name which for the first time shows how we can create these force sensitive stickers (Fig. \ref{fig:intro_fig}a,b), which can be stuck to everyday objects (Fig. \ref{fig:intro_fig}c), as well as flexibly confirm to orthopaedic implants (Fig. \ref{fig:intro_fig}d) and robots (Fig. \ref{fig:intro_fig}e), in order to meet these various applications.
\name solves three challenges to create such force sensitive stickers.
First, \name designs a 0.4mm thick force sensor which utilizes a novel force transduction mechanism that alters the wireless channel at Radio Frequencies (RF) as the sensor deforms under applied forces.
This transduction mechanism allows for measurable changes in wireless channel even though the sensor deformations are sub-mm level, which creates a powerful joint communication sensing paradigm with a mm-scale force sensor.
Second, to achieve the sticker form factor and modulate the sensor signals for wireless detection, we interface these mm-scale force sensors to UHF RFID stickers.
Thus we measure the force by observing channel estimates given by RFID readers for each sensor interfaced RFID tag.
Finally, we create robust signal processing algorithms to allow for reliable wireless force sensing in variety of environments, and even in presence of moving multipath, to achieve the vision of ubiquitous force sensing.

The first challenge in creation of such force sensitive stickers is the mm-scale sensor fabrication and the associated transduction mechanism. 
% Previous work \cite{} has used a linear relationship between contact length effect created by force formation versus the wireless channel phase for transduction mechanism.
The requirements from the transduction mechanism would be to create measurable changes in wireless channel to enable joint communication sensing ability.
However, with a mm-scale sensor, the deformations caused by applied forces would be further sub-mm, which pose a challenge to create any measurable wireless channel changes.
For instance, if a simple linear deformation to phase change transduction is used, with a 0.1mm deformation, the net wireless channel phase would only change by 0.1 degrees, not enough to be measurable at the RFID reader~\cite{}. 
Instead, \name proposes a new transduction mechanism between load capacitances and phase change, which enable a non-linear relationship between deformation and wireless channel changes. 
This transduction mechanism is similar to how varactors create phase shifts in RF circuits.
Essentially, \name designs a mm-scale force sensitive varactor sensor at 900 MHz, which gives measurable phase changes even when the sensor is miniaturized. We perform multiphysics simulations in order to solve both maxwell's equations for force impedance calculations, as well as solid mechanics equations for force deformation in order to understand the transduction phenomenon and design the sensor appropriately to guarantee a measurable wireless channel phase change for the joint communication sensing paradigm proposed by \name.

The second challenge is how do we interface the fabricated sensor with RFIDs, in order to modulate the phase shifted signals from the sensor so that the remotely located reader can discern the sensor reflection from the other signals it receives. 
A naive approach could be to cut a small piece of the RFID antenna and attach the sensor between the cut pieces. 
However, this approach severly impacts the RFID range and the readings becoem unreliable~\cite{}.
In comparison, \name makes a key observation that the \name sensor is purely capacitative, and thus has purely reactive impedance. 
When a purely reactive impedance is interfaced in parallel to the RFIDs, we obtain a pure phase shifted signal with no changes in magnitude. 
To do so, we interface \name's sensor to COTS RFID stickers via two 20$\mu$m tungsten wire filaments, and show that this interfacing does not impact the RFID range.
Thus, it creates robust RFID modulated and phase shifted reflections from the sensor.
In addition to COTS RFID stickers, we also show a possible interfacing method of the sensor by creating a PCB pad for the sensor, similar to how capacitors have standard size pads (0603, 0805 etc) for PCB based interfacing. 
In addition This allows \name to also create custom RFID tags on flexible PCB substrates, and we utilize a self designed small antenna to further miniaturize the form factor of the sensor and showcase possible interfacing with other backscatter ICs in addition to RFIDs. 

% The third challenge is signal processing algorithms..phase variations: delta phase as a reliable metric
Finally, we design novel signal processing algorithms to read the phase changes from the sensor, via phase readings reported by the RFID reader. FCC compliant RFID readers hop across the 900-930 MHz RFID band every 200ms, which creates phase discontinuities in the reported phase. However, since \name sensor conveys the force information via change of phases, by taking differential phases we can get rid of the random hopping offsets introduced.
Further, we can get accurate to 1 degree phase readings by performing averaging across the 50 channels of RFID operation, which allows for robust wireless force sensing.
We also test the sensor with people moving around and show the robustness of phase sensing to the dynamic multipath as well.

Hence, to summarize, we first design the mm-scale sensors which work successfully at RF frequencies and integrate them with flexible RFIDs to attain the sticker form factor batteryless force sensors.
The sensor by itself is 1000x lower volume form factor as compared to recent past work ~\cite{} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained are consistent with the porposed transuction mechanism of capacitance to phase changes via FEM multiphysics simulations in COMSOL. Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model.
% Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications


==> intros/introv6_0.tex <==
% !TEX root = paper.tex

\section{Introduction}
% \begin{itemize}[leftmargin=0pt]
%     \item \textbf{All objects/human interactions happen due to contact force, sensing forces ubiquitously can capture and quantify/digitize a lot of information about environment}
%     \item \textbf{However, this requires a force sensor which can be stuck around without disturbing the environment in the first place; it should confirm well to uneven surfaces and not require wires}
%     \item \textbf{Not only ubiquitous sensing, such sticker-like sensors will also enable new medical applications which also require similar batteryless sensing approaches}
%     \item \textbf{We present \name which is the first such sensor to achieve these applications.. }
%     \item \textbf{Our key insight is to design a <1mm thick miniaturized capacitive force sensor at 900 MHz RFID frequencies, where it acts akin to a force sensitive varactor}
%     \item \textbf{The force sensitive varactor design creates changes in wireless channel by shifting signal phases due to application of force, which is utilized to read the sensor wirelessly}
%     \item  \textbf{We simulate the sensor in a multiphysics simulator to confirm it's working at 900 MHz. 
%     Further, we also show how sensor can be integrated with existing RFID backscatter systems to allow for wireless operation}
%     \item \textbf{We also show how to have the sensor as a PCB component with a designed PCB pad for easy interfacing with antennas and ICs. We also show a small antenna designs to improve on the form factor}
%     \item \textbf{Finally, we build algorithms to sense phase from RFID reader reliably to sense the force robustly}
%     \item \textbf{Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications}
% \end{itemize}

% Force ubiquiti
\noindent Force is an ubiquitous phenomenon in our daily environment, with there being gravitational contact force exerted by any object's weight onto it's support, our range of daily activities involving various interaction forces between various bone joints and ligaments, among so many other static, as well as motile scenarios where various actors in the environment apply forces on each other. However, a lack of ubiquitously available force sensors lead to these interactions not being recorded and quantified, creating a big gap between our digital world and the real environment.

Ability to quantify these force interactions would open the door to myriad of applications. For example, if we could sense the weight of packages in a warehouse setting, we can use it for integrity check~\cite{}, since an empty or improperly packed package would apply a lower gravitational force. Today, we have 3-D printed orthopaedic implants for knee-replacement surgeries. An implant equipped with a force sensor could measure the contact forces between the knee joints as the patient recovers post-surgery to categorize the implant health and how well the body accepts the knee implant~\cite{}. Another application area is robotics, where these force sensors can be used to better control the robots, for example while gripping a sensitive objects the robotic manipulator needs to quantify the forces it is applying~\cite{}, and in surgical robots which have to be careful while interacting with body tissues so that they don't damage the tissues by applying excessive forces~\cite{}. 
% in field of surgical robots which navigate in tight in-vivo spaces where the robot can 

These applications pose numerous challenges, and hence are not mainstream today.
In order to ubiquitously sense weight in warehouse settings, we need to create force sensors which can be simply stuck to the bottom of the packages like a barcode and be read wirelessly to measure the weight of the contents.
Such sensors, if made miniaturized enough and flexible, can also confirm to the uneven shapes of orthopaedic implants and read the bone joint forces.
In addition to form-factor and flexibility requirements, such in-vivo applications would also require batteryless operation, since we can not have risk of contamination by carrying small coin cell batteries inside the body.
Further, such battery-free wireless force stickers can fulfill robotic applications which also require force sensors to be mount in unusual space constraint places. 
With today's force sensing technologies, most of them being wired, or requiring batteries, fabricating such force-sensitive stickers is impossible and hence these applications remain hypothetical and researched in laboratory settings only.

In this paper, we present \name which for the first time shows how we can create these force sensitive stickers, which can be stuck to everyday objects, as well as flexibly confirm to orthopaedic implants and robots, in order to meet these various applications.
\name solves three challenges to create such force sensitive stickers.
First, \name designs a 0.4mm thick force sensor which utilizes a novel force transduction mechanism that alters the wireless channel at Radio Frequencies (RF) as the sensor deforms under applied forces.
This transduction mechanism allows for measurable changes in wireless channel even though the sensor deformations are sub-mm level, which creates a powerful joint communication sensing paradigm with a mm-scale force sensor.
Second, to achieve the sticker form factor and modulate the sensor signals for wireless detection, we interface these mm-scale force sensors to UHF RFID stickers.
Thus we measure the force by observing channel estimates given by RFID readers for each sensor interfaced RFID tag.
Finally, we create robust signal procssing algorithms to allow for reliable wireless force sensing in variety of environments, and even in presence of moving multipath, to achieve the vision of ubiquitous force sensing.

The first challenge in creation of such force sensitive stickers is the sensor fabrication and the associated transduction mechanism. Previous work \cite{} has used a linear relationship between contact length effect created by force formation versus the wireless channel phase for transduction mechanism.
Such transduction mechanism prohibit the sensor to get miniaturized to mm-scale, since at these RFID frequencies of 900 MHz, the maximum phase change available via 1mm deformation would be 1 degree, not enough to be measurable at the RFID reader. Instead, \name proposes a new transduction mechanism, based on a non-linear relationship between load capacitances and phase change, used in today's varactors to create phase shifts. Essentially, \name designs a mm-scale force sensitive varactor sensor at 900 MHz, which gives measurable phase changes even when the sensor is miniaturized. We perform multiphysics simulations in order to solve both maxwell's equations for force impedance calculations, as well as solid mechanics equations for force deformation in order to guarantee a measurable wireless channel phase change for the joint communication sensing paradigm proposed by \name.

The second challenge is how do we interface the sensor with RFIDs, in order to modulate the phase shifted signals from the sensor so that the remotely located reader can discern the sensor reflection from the other signals it receives. A previous work \cite{} tries to interface COTS pressure sensors with RFIDs by cutting a small piece of the RFID antenna and attaching the sensor between the cut pieces. However, this approach severly impacts the RFID range and the readings becoem unreliable.
In comparison, \name makes a key observation that the \name sensor is purely capacitative, and thus has purely reactive impedance. When a purely reactive impedance is interfaced in parallel to the RFIDs, we obtain a pure phase shifted signal with no changes in magnitude. Hence, interfacing the \name sensor to RFIDs does not impact the RFID range.
Further, we show a possible interfacing method of the sensor by creating a PCB pad for the sensor, similar to how capacitors have standard size pads (0603, 0805 etc) fo PCB based interfacing. 
This allows \name to also create custom RFID tags on flexible PCB substrates, and we utilize a self designed small antenna to further miniaturize the form factor of the sensor and showcase possible interfacing with other backscatter ICs in addition to RFIDs. 

% The third challenge is signal processing algorithms..phase variations: delta phase as a reliable metric
Finally, we design novel signal processing algorithms to read the phase changes from the sensor, via phase readings reported by the RFID reader. FCC compliant RFID readers hop across the 900-930 MHz RFID band every 200ms, which creates phase discontinuities in the reported phase. However, since \name sensor conveys the force information via change of phases, by taking differential phases we can get rid of the random hopping offsets introduced.
Further, we can get accurate to 1 degree phase readings by performing averaging across the 50 channels of RFID operation, which allows for robust wireless force sensing.
We also test the sensor with people moving around and show the robustness of phase sensing to the dynamic multipath as well.

Hence, to summarize, we first design the mm-scale sensors which work successfully at RF frequencies and integrate them with flexible RFIDs to attain the sticker form factor batteryless force sensors.
The sensor by itself is 1000x lower volume form factor as compared to recent past work ~\cite{} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained are consistent with the porposed transuction mechanism of capacitance to phase changes via FEM multiphysics simulations in COMSOL.Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model.
% Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications


==> intros/introv7.tex <==
% !TEX root = paper.tex
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{intros/introv6_fig_1.pdf}
    \caption{(a) Shows the 2 versions of \name (b) demonstrates the flexibility of the sensors (c) shows how \name can be stuck on bottom of packages to measure the weight of contents inside for integrity checks (d) shows how \name can be used for in-vivo implant force sensing and (e) shows a possible integration of \name sensor with tendon driven robots}
    \label{fig:intro_fig}
\end{figure}
\section{Introduction}
% \begin{itemize}[leftmargin=0pt]
%     \item \textbf{All objects/human interactions happen due to contact force, sensing forces ubiquitously can capture and quantify/digitize a lot of information about environment}
%     \item \textbf{However, this requires a force sensor which can be stuck around without disturbing the environment in the first place; it should confirm well to uneven surfaces and not require wires}
%     \item \textbf{Not only ubiquitous sensing, such sticker-like sensors will also enable new medical applications which also require similar batteryless sensing approaches}
%     \item \textbf{We present \name which is the first such sensor to achieve these applications.. }
%     \item \textbf{Our key insight is to design a <1mm thick miniaturized capacitive force sensor at 900 MHz RFID frequencies, where it acts akin to a force sensitive varactor}
%     \item \textbf{The force sensitive varactor design creates changes in wireless channel by shifting signal phases due to application of force, which is utilized to read the sensor wirelessly}
%     \item  \textbf{We simulate the sensor in a multiphysics simulator to confirm it's working at 900 MHz. 
%     Further, we also show how sensor can be integrated with existing RFID backscatter systems to allow for wireless operation}
%     \item \textbf{We also show how to have the sensor as a PCB component with a designed PCB pad for easy interfacing with antennas and ICs. We also show a small antenna designs to improve on the form factor}
%     \item \textbf{Finally, we build algorithms to sense phase from RFID reader reliably to sense the force robustly}
%     \item \textbf{Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications}
% \end{itemize}

% Force ubiquiti
\noindent Force is an ubiquitous phenomenon in our daily environment, with any two objects in contact exerting forces onto each other.
In case of an object in contact with a table, there would be the objects weight (gravitational force) exerted onto the table.
Another example of two objects in contact could be our bone joints, which create movement by exerting the interaction forces on the other bones and ligaments in contact via the joint.
Force sensors can quantify these ubiquitous contact phenomenon, and bridge the gap between the digital world and the real environment.

% Any object would exert it's weight (gravitational force) onto it's support, and our range of daily activities involves various interaction forces between various bone joints and ligaments, among various other examples. 
% % However, a lack of ubiquitously available force sensors lead to these interactions not being recorded and quantified, creating a big gap between our digital world and the real environment.

Hence, force sensors enable myriad of applications, in diverse fields like warehouse scenarios, orthopaedic implants and robotics.
For example, we could sense the weight of packages in a warehouse setting, and then use it for integrity checks~\cite{sensor_checking_weights}, since an empty or improperly packed package would apply a lower gravitational force. 
Similarly, an orthopaedic implant equipped with a force sensor could measure the contact forces between the knee joints as the patient recovers post-surgery to categorize the implant health and how well the body accepts the knee implant~\cite{sensor_check_knee_implants_1,sensor_check_knee_implants_2}. 
Another application area is robotics, where these force sensors can be used to better control the robots, for example while gripping a sensitive objects the robotic manipulator needs to quantify the forces it is applying~\cite{gripper_force_needed_1_fruit,gripper_force_needed_2_robotic}, and in surgical robots which have to be careful while interacting with body tissues so that they don't damage the tissues by applying excessive forces~\cite{force_needed_1_surgical_robot}. 
% in field of surgical robots which navigate in tight in-vivo spaces where the robot can 

However, these applications pose numerous challenges, and hence are not mainstream today.
In order to ubiquitously sense weight in warehouse settings, requiring a full-fledged weighing scale below the packages to measure weight won't be practical, and hence we need to create force sensors which can be simply stuck to the bottom of the packages like a barcode and be read wirelessly to measure the weight of the contents.
Further, such sensors, if made miniaturized enough and flexible, can also confirm to the uneven shapes of orthopaedic implants and read the bone joint forces.
In addition to form-factor and flexibility requirements, such in-vivo applications would also require batteryless operation, since we can not have risk of contamination by carrying small coin cell batteries inside the body.
Further, such battery-free wireless force stickers can fulfill robotic applications which also require force sensors to be mount in unusual space constraint places. 
With today's force sensing technologies, most of them being wired, or requiring batteries, fabricating such force-sensitive stickers is impossible and hence these applications remain hypothetical and researched in laboratory settings only to show potential benefits of force sensing, hence force sensors aren't a ubiquitous part of our daily life.

In this paper, we present \name which for the first time shows how we can create these force sensitive stickers (Fig. \ref{fig:intro_fig}a,b), which can be stuck to everyday objects (Fig. \ref{fig:intro_fig}c), as well as flexibly confirm to orthopaedic implants (Fig. \ref{fig:intro_fig}d) and robots (Fig. \ref{fig:intro_fig}e), in order to meet these various applications.
\name has three design components central to the creation of such force sensitive stickers, introduction of a new transduction mechanism which maps applied forces to wireless signal fluctuations, 
designing a mm-scale sensor which harnesses the new transduction mechanism and
interfacing the fabricated sensors to RFIDs for batteryless and wireless operation.

% First, \name designs a 0.4mm thick force sensor which utilizes a novel force transduction mechanism that directly alters the Radio Frequencies (RF) wireless signals as the sensor deforms under applied forces.
% This transduction mechanism allows for wirelessly measurable changes at a remotely located radio which receives these altered wireless signals reflecting off from the sensor.
% The key contribution here is that even though the sensor faces deformations which are sub-mm level due to applied forces, the effects of this tiny sub-mm deformations can be sensed as far as 5m away without requiring any sort of battery.
% Second, to achieve the sticker form factor and modulate the sensor signals for wireless detection, we interface these mm-scale force sensors to RFID stickers.
% Thus we can measure the forces by observing channel estimates given by RFID readers for each sensor interfaced RFID tag, and these channel estimates contain the information of wireless signal alterations due to force transduction.
% Finally, we create robust signal processing algorithms to allow for reliable wireless force sensing in variety of environments, and even in presence of moving multipath, to achieve the vision of ubiquitous force sensing.

The first design component in creation of such force sensitive stickers is the associated transduction mechanism which creates the alterations in wireless signals reflecting off from the sensor due to applied forces.
Although there exist mm-scale discrete force sensors today, these sensors typically create small voltage fluctuations which needs to be sensed either locally via amplifiers and ADCs, or be communicated via wires, which prevent usage of these sensors in a batteryless sticker-like form factor sensing system.
In comparison, \name's approach of force transduction avoids these issues by creating fluctuations which can travel via the wireless signals to a remotely located reader, and not requiring local measurement electronics like ADCs or wires.
This mechanism effectively communicates information by creating fluctuations in the wireless channel between the reader and the sensor.
% Previous work \cite{} has used a linear relationship between contact length effect created by force formation versus the wireless channel phase for transduction mechanism.
Henceforth, the requirements from this transduction mechanism would be to create measurable changes in wireless channel.
It is indeed challenging to consider how small sub-mm deformations caused by applied forces create substantial signal fluctuations to be read off by a remotely located reader robustly in presence of all the environmental clutter and noise.
% However, with a mm-scale sensor, the deformations caused by applied forces would be further sub-mm, which pose a challenge to create any measurable wireless channel changes.
For instance, past work \cite{} which also tries to achieve the similar transduction, by creating wireless signal phase shifts due to applied forces required a 80mm long sensor to create $12^{o}$ phase change via a linear phase to length relationship.
If this sensor is naively miniaturized to even $10mm$, the total phase change would get $1.5^{o}$ which is not enough to be measurable at the reader~\cite{}. 

Instead, \name proposes a new transduction mechanism between load capacitances and RF phase change, which essentially enables a measurable $>10^{o}$ phase change, from the sub-mm deformations, even when the sensor is miniaturized to mm-scale.
This creates a power joint communication-sensing paradigm for force sensors that can scale to mm-scale sensors, since the phase shift based sensing mechanism also can get communicated to remotely located reader simultaneously.
% This transduction mechanism is similar to how varactors create phase shifts in RF circuits.
% Essentially, \name designs a mm-scale force sensitive varactor sensor at 900 MHz, which gives measurable phase changes even when the sensor is miniaturized. 
We provide a mathematical understanding of this new transduction mechanism and show how to design such capacitive force sensors which transduce force to RF signal phases.
Further, we perform multiphysics simulations in order to solve both maxwell's equations for force impedance calculations, as well as solid mechanics equations for force deformation in order to model the transduction phenomenon and confirm the sensor design, as well as the required RF interfacing, to guarantee a measurable wireless channel phase change for the joint communication sensing paradigm proposed by \name.

The second design component of \name is how do we interface the fabricated sensor with RFIDs, in order to modulate the phase shifted signals from the sensor so that the remotely located reader can discern the sensor reflection from the other signals it receives. 
A naive approach could be to cut a small piece of the RFID antenna and attach the sensor between the cut pieces. 
However, this approach severly impacts the RFID range and the readings become unreliable~\cite{}.
% In comparison, \name makes a key observation that the \name sensor is purely capacitative, and thus has purely reactive impedance. 
In comparison, \name makes a key observation that the \name sensor is designed to be purely capacitative, and thus has purely reactive impedance. 
When a purely reactive impedance is interfaced in parallel to the RFIDs, we obtain a pure phase shifted signal with no changes in magnitude. 
Since \name sensor only affects phase and not magnitude, it does not disturb the operation of RFID energy harvestor and hence does not disturb the RFID reading range.
% To do so, we interface \name's sensor to COTS RFID stickers via two 20$\mu$m tungsten wire filaments, and show that this interfacing does not impact the RFID range.
% Thus, it creates robust RFID modulated and phase shifted reflections from the sensor.
This interfacing with RFIDs without losing any range allows for robust wireless sensing which does not compromise the reading range, or the sensor signal strength.
% In addition to COTS RFID stickers, we also show a possible interfacing method of the sensor by creating a PCB pad for the sensor, similar to how capacitors have standard size pads (0603, 0805 etc) for PCB based interfacing. 
In addition \name also creates custom RFID tags on flexible PCB substrates, and we utilize a self designed small 1cm$\times$1cm spiral PCB printed antenna to further miniaturize the form factor of the sensor.
We also show how we can interface the \name sensor with existing commercialized RFID strickers in a standalone manner without requiring a PCB.

% The third challenge is signal processing algorithms..phase variations: delta phase as a reliable metric go slow here RFID reading
% todo for tomorrow: design choice enables robust reading 
Finally, we design novel signal processing algorithms to read the phase changes from the sensor, via phase readings reported by the RFID reader. FCC compliant RFID readers hop across the 900-930 MHz RFID band every 200ms, which creates phase discontinuities in the reported phase. However, since \name sensor conveys the force information via change of phases, by taking differential phases over time, we can get rid of the random hopping offsets introduced.
This elimination of random phase offsets allows for collating consistent information across the 50 different RFID channels, which in turn allows improved sensing performance because of channel averaging of phases, giving the capability to read phase changes accurate to 0.5-1 degree, which allows to sense forces with 0.2-0.4 N resolution across the 0-6N sensing range.
We also test the sensor with people moving around and show the robustness of phase sensing to the dynamic multipath as well.

Hence, to summarize, we first design the mm-scale sensors which work successfully at RF frequencies and integrate them with flexible RFIDs to attain the sticker form factor batteryless force sensors.
The sensor by itself is 1000x lower volume form factor as compared to recent past work ~\cite{wiforce} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained are consistent with the proposed transduction mechanism of capacitance to phase changes via FEM multiphysics simulations in COMSOL. Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 10000 contact points, both over the air and over a pork belly setup for in-body sensing. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model.
% Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications


==> intros/introv8.tex <==
% !TEX root = paper.tex
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{intros/introv6_fig_1.pdf}
    \caption{(a) Shows the 2 versions of \name (b) demonstrates the flexibility of the sensors (c) shows how \name can be stuck on bottom of packages to measure the weight of contents inside for integrity checks (d) shows how \name can be used for in-vivo implant force sensing and (e) shows a possible integration of \name sensor with tendon driven robots}
    \label{fig:intro_fig}
\end{figure}
\section{Introduction}
% \begin{itemize}[leftmargin=0pt]
%     \item \textbf{All objects/human interactions happen due to contact force, sensing forces ubiquitously can capture and quantify/digitize a lot of information about environment}
%     \item \textbf{However, this requires a force sensor which can be stuck around without disturbing the environment in the first place; it should confirm well to uneven surfaces and not require wires}
%     \item \textbf{Not only ubiquitous sensing, such sticker-like sensors will also enable new medical applications which also require similar batteryless sensing approaches}
%     \item \textbf{We present \name which is the first such sensor to achieve these applications.. }
%     \item \textbf{Our key insight is to design a <1mm thick miniaturized capacitive force sensor at 900 MHz RFID frequencies, where it acts akin to a force sensitive varactor}
%     \item \textbf{The force sensitive varactor design creates changes in wireless channel by shifting signal phases due to application of force, which is utilized to read the sensor wirelessly}
%     \item  \textbf{We simulate the sensor in a multiphysics simulator to confirm it's working at 900 MHz. 
%     Further, we also show how sensor can be integrated with existing RFID backscatter systems to allow for wireless operation}
%     \item \textbf{We also show how to have the sensor as a PCB component with a designed PCB pad for easy interfacing with antennas and ICs. We also show a small antenna designs to improve on the form factor}
%     \item \textbf{Finally, we build algorithms to sense phase from RFID reader reliably to sense the force robustly}
%     \item \textbf{Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications}
% \end{itemize}

% Force ubiquiti
\noindent Force is an ubiquitous phenomenon in our daily environment, with any two objects in contact exerting forces onto each other. Therefore, force sensors are a simple and unique way to quantify ubiquitous contact phenomenon, and bridge the gap between the digital world and the real environment, with clear use cases in AR/VR and ubiquitous computing\cite{}. Further, these force sensors can enable myriad of diverse applications, from warehouse scenarios, orthopaedic implants to robotics.
For example, we could sense the weight (force) of the packages in a warehouse setting, and use the sensed force for integrity of the packages~\cite{sensor_checking_weights}, since an empty or improperly packed package would apply a lower gravitational force. Similarly, an orthopaedic implant equipped with a force sensor could measure the contact forces between the knee joints as the patient recovers post-surgery to categorize the implant health (shown in Fig.xx) and how well the body accepts the knee implant~\cite{sensor_check_knee_implants_1,sensor_check_knee_implants_2}. Another application area is robotics, where these force sensors can be used to better control the robots, for example while gripping a sensitive objects the robotic manipulator needs to quantify the forces it is applying~\cite{gripper_force_needed_1_fruit,gripper_force_needed_2_robotic}, and in surgical robots which have to be careful while interacting with body tissues so that they don't damage the tissues by applying excessive forces~\cite{force_needed_1_surgical_robot}. 
% in field of surgical robots which navigate in tight in-vivo spaces where the robot can 

However, these applications pose numerous challenges on force sensors, and hence the applications are not mainstream today. 
For example, consider the usecase of sensing forces sustained by the knee-implant.
In this scenario, the force sensors need to be thin enough to fit within the narrow gaps between the bones in the knee joint.
Further it needs to fit snugly to the uneven bone shapes in the knee joint.
Since the implant is located inside the body (in-vivo), it is not possible to carry a wire till the sensor, and thus the sensor has to be read wirelessly via a remotely located reader outside the body.
To enable wireless operation, we can not assume an active radio near the sensor to transmit the sensor readings, since batteries pose a risk of contamination inside body, as well as requirement of battery would not allow for thin sticker-like sensors.
Hence, the most ideal force sensor has to be somehow thin and sticker-like form factor to fit snugly inside the joint, and at the same time support wireless operation without requiring a battery.
% Further it need to flex and fit snugly to the uneven bone shapes in the knee joint.
% In order to ubiquitously sense weight (force) in warehouse settings, requiring a full-fledged weighing scale below the packages to measure weight, which won't be practical. A natural question is can we create force sensors which are `passive' stickers like a barcode, that can be simply attached to the bottom of the packages and be read `wirelessly' to measure the weight of the contents.
% Further, if such sensors, if made `minute enough and flexible', can also conform to the uneven shapes of orthopaedic implants and read the bone joint forces.
% In addition to form-factor and flexibility requirements, such in-vivo applications would also require `batteryless' operation, since we can not have risk of contamination by carrying small coin cell batteries inside the body.
% Further, such battery-free wireless force stickers can fulfill robotic applications which also require force sensors to be mount in unusual space constraint places. 
% With today's force sensing technologies, most of them being wired, or requiring batteries, fabricating such force-sensitive stickers is impossible and hence these applications remain hypothetical and researched in laboratory settings only to show potential benefits of force sensing, hence force sensors aren't a ubiquitous part of our daily life.

In this paper, we present \name which for the first time demonstrates these wireless force sensitive stickers (Fig. \ref{fig:intro_fig}a,b), which can be stuck to everyday objects (Fig. \ref{fig:intro_fig}c), as well as flexibly confirm to orthopaedic implants (Fig. \ref{fig:intro_fig}d) and robots (Fig. \ref{fig:intro_fig}e), in order to meet these various applications. 
Specifically, \name develops a novelforce sensitive sensor, which are mm-scale as shown in Fig. xx, and are energy efficient.
% , and develops a novel force transduction mechanism that directly alters the Radio Frequencies (RF) wireless signals as the sensor deforms under applied forces. 
Furthermore, \name uniquely interfaces these mm-scale force sensors to RFID stickers, which is not only flexible sticker, but also allows for wireless interrogation of sensor via a remotely located RFID reader, similar to how barcodes are read wirelessly via barcode scanners, without requiring a battery at the barcode.
% This integration allows \name's flexible, mm-scaled, energy efficient force sensor to use the popular battery-free RFID backscatter modulation to achieve wireless communication without requiring a battery.
% also achieves wireless communication in a battery-free manner. 
% performance as RFID tags, but can modulate the sensor signals for wireless reading.
\name finally develops robust signal processing algorithms atop of the COTS RFID reader, to allow for reliable reading of applied forces on the mm-scale sensor, in variety of environments, and even in presence of moving objects in the environment, to achieve the vision of ubiquitous force sensing. 
This method of creating force sensitive RFID stickers easily meets the motivated applications of knee implant force sensing and ubiquitous weight sensing in warehouses, as well as have the potential to enable many more applications.
% The key insight behind \name's flexible, mm-scaled, energy efficient force sensor design is that the sensor basically encodes force information directly onto the RFID modulated wireless signals reflecting off from the sensor, integrated with popular battery-free RFID backscatter modulation gives a can easily meet xyz applications...  Furthermore, \name stickers has potential to enable many more applications. 

The first design element of \name is to develop the energy efficient force sensitive sensor, which are mm-sized and transmutes the applied force easily to wireless technologies. 
Although there exist mm-scale discrete force sensors today, these sensors typically create small voltage fluctuations which needs to be sensed locally via amplifiers and ADCs, which prevent usage of these sensors to be energy efficient, and hence cannot be used in a batteryless sticker-like form factor. 
In comparison, \name's approach of force transduction avoids these issues by directly creating fluctuations on reflections components of the signals travelling  to and fro the remotely located RFID reader.
The RFID reader measures these fluctuations in the reflected signal caused by the applied forces on the sensor, and hence this technique does not not requires local measurement electronics like ADCs or wires near the sensor, and hence the sensor can be battery-free. 
The overall technique is again similar to a barcode scanner, which illuminates the barcode with laser light selectively reflected by the white portions on the barcode, hence the barcode information is encoded onto the reflections bouncing off from the barcode.
However, in case of the \name sensor, the force information is encoded onto the reflected signal instead of just the barcode information.

A recent work attempts the similar transduction, by creating wireless signal phase shifts due to applied forces; It required a large sensor (80mm), to create measurable channel change. More specifically the sensor length (size) is proportional to the changes in the channel. Therefore, it is make challenging to create a small sub-mm sized sensor, on which deformations caused by applied forces create substantial signal fluctuations to be read off by a remotely located reader robustly in presence of all the environmental clutter and noise.

Instead, \name proposes a new transduction mechanism instead of length of the sensor, it develops a new mechanism using the capacitances. Specifically, \name develops a new transduction mechanism translating the load capacitance into RF phase change even at RF frequencies, which essentially enables a measurable $>10^{o}$ phase change, from the sub-mm deformations, even when the sensor is miniaturized to mm-scale.
% This transduction mechanism is similar to how varactors create phase shifts in RF circuits.
% Essentially, \name designs a mm-scale force sensitive varactor sensor at 900 MHz, which gives measurable phase changes even when the sensor is miniaturized. 
We provide a mathematical understanding of this new transduction mechanism and show how to design such capacitive force sensors which transduces force to RF signal phases.
Further, we perform multiphysics simulations in order to solve both maxwell's equations for force impedance calculations, as well as solid mechanics equations for force deformation in order to model the transduction phenomenon and confirm the sensor design, as well as the required RF interfacing, to guarantee a measurable wireless channel phase change for the joint communication sensing paradigm proposed by \name. Thus, \name creates a power joint communication-sensing paradigm for force sensors that can scale to mm-scale sensors, and would be energy efficient, and modulate the RF signals with a phase shift proportional to applied force.
 
% \name has three design components central to the creation of such force sensitive stickers, introduction of a new transduction mechanism which maps applied forces to wireless signal fluctuations, 
% designing a mm-scale sensor which harnesses the new transduction mechanism and
% interfacing the fabricated sensors to RFIDs for batteryless and wireless operation.


% This mechanism effectively communicates information by creating fluctuations in the wireless channel between the reader and the sensor.
% Previous work \cite{} has used a linear relationship between contact length effect created by force formation versus the wireless channel phase for transduction mechanism.
% Henceforth, the requirements from this transduction mechanism would be to create measurable changes in wireless channel.

% However, with a mm-scale sensor, the deformations caused by applied forces would be further sub-mm, which pose a challenge to create any measurable wireless channel changes.

% If this sensor is naively miniaturized to even $10mm$, the total phase change would get $1.5^{o}$ which is not enough to be measurable at the reader~\cite{}. 



Next, we design an interface for \name sensor to the backscatter technology like RFIDs, which can directly modulate the force-to-phase shift onto the wireless channel of RFID tags and enable battery-free operation. Furthermore, it would also enable \name to support multiple force sensors concurrently as well, with RFID providing unique identity. Previous efforts have attempted RFID based sensor integration, cut a small piece of RFID antenna and installed a sensor, which inadvertently lead to reduced range of operation and the readings become unreliable~\cite{}. 
% in order to modulate the phase shifted signals from the sensor so that the remotely located reader can discern the sensor reflection from the other signals it receives. 
% A naive approach could be to cut a small piece of the RFID antenna and attach the sensor between the cut pieces. 
% In comparison, \name makes a key observation that the \name sensor is purely capacitative, and thus has purely reactive impedance. 
In comparison, \name makes a key observation that the \name sensor is designed to be purely capacitative, and thus has purely reactive impedance. 
When a purely reactive impedance is interfaced in parallel to the RFIDs, we obtain a pure phase shifted signal with no reduction in the magnitude of reflected signal.
Since \name sensor only affects phase and not magnitude, it does not disturb the operation of RFID energy harvestor and hence does not reduce the RFID reading range.
% To do so, we interface \name's sensor to COTS RFID stickers via two 20$\mu$m tungsten wire filaments, and show that this interfacing does not impact the RFID range.
% Thus, it creates robust RFID modulated and phase shifted reflections from the sensor.
This interfacing with RFIDs without losing any range allows for robust wireless sensing which does not compromise the reading range, or the sensor signal strength.
% In addition to COTS RFID stickers, we also show a possible interfacing method of the sensor by creating a PCB pad for the sensor, similar to how capacitors have standard size pads (0603, 0805 etc) for PCB based interfacing. 
In addition \name also creates custom RFID tags on flexible PCB substrates, and we utilize a self designed small 1cm$\times$1cm spiral PCB printed antenna to further miniaturize the form factor of the sensor.
We also show how we can interface the \name sensor with existing commercialized RFID strickers in a standalone manner without requiring a PCB.

% The third challenge is signal processing algorithms..phase variations: delta phase as a reliable metric go slow here RFID reading
% todo for tomorrow: design choice enables robust reading 
Finally, we design novel signal processing algorithms to read the phase changes from the sensor using COTS RFID readers, which would enable immediately usablity of \name. \name develops the force measurement via phase readings reported by the RFID reader. FCC compliant RFID readers hop across the 900-930 MHz RFID band every 200ms, which creates phase discontinuities in the reported phase. However, since \name sensor conveys the force information via change of phases, by taking differential phases over time, we can get rid of the random hopping offsets introduced.
This elimination of random phase offsets allows for collating consistent information across the 50 different RFID channels, which in turn allows improved sensing performance because of channel averaging of phases, giving the capability to read phase changes accurate to 0.5-1 degree, which allows to sense forces with 0.2-0.4 N resolution across the 0-6N sensing range.
We also test the sensor with people moving around and show the robustness of phase sensing to the dynamic multipath as well.

Hence, to summarize, we first design the mm-scale sensors which work successfully at RF frequencies and integrate them with flexible RFIDs to attain the sticker form factor batteryless force sensors.
The sensor by itself is 1000x lower volume form factor as compared to recent past work ~\cite{wiforce} on wireless force sensors and is the first work to showcase an end-to-end batteryless wireless operation.
We also confirm that the experimental results obtained are consistent with the proposed transduction mechanism of capacitance to phase changes via FEM multiphysics simulations in COMSOL. Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 10000 contact points, both over the air and over a pork belly setup for in-body sensing. We also motivate two application case studies with our sensor, with first case study involved with putting these sensors on robots and sensing the applied robot force and the second usecase showing how we can read the forces applied by knee joints via a toy-knee model. \todo{more strongly...}
% Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications


==> intros/introv9.tex <==
% !TEX root = paper.tex
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{intros/introv6_fig_1.pdf}
    \caption{(a) Shows the 2 versions of \name (b) demonstrates the flexibility of the sensors (c) shows how \name can be stuck on bottom of packages to measure the weight of contents inside for integrity checks (d) shows how \name can be used for in-vivo implant force sensing and (e) shows a possible integration of \name sensor with tendon driven robots}
    \label{fig:intro_fig}
\end{figure}
\section{Introduction}
% \begin{itemize}[leftmargin=0pt]
%     \item \textbf{All objects/human interactions happen due to contact force, sensing forces ubiquitously can capture and quantify/digitize a lot of information about environment}
%     \item \textbf{However, this requires a force sensor which can be stuck around without disturbing the environment in the first place; it should confirm well to uneven surfaces and not require wires}
%     \item \textbf{Not only ubiquitous sensing, such sticker-like sensors will also enable new medical applications which also require similar batteryless sensing approaches}
%     \item \textbf{We present \name which is the first such sensor to achieve these applications.. }
%     \item \textbf{Our key insight is to design a <1mm thick miniaturized capacitive force sensor at 900 MHz RFID frequencies, where it acts akin to a force sensitive varactor}
%     \item \textbf{The force sensitive varactor design creates changes in wireless channel by shifting signal phases due to application of force, which is utilized to read the sensor wirelessly}
%     \item  \textbf{We simulate the sensor in a multiphysics simulator to confirm it's working at 900 MHz. 
%     Further, we also show how sensor can be integrated with existing RFID backscatter systems to allow for wireless operation}
%     \item \textbf{We also show how to have the sensor as a PCB component with a designed PCB pad for easy interfacing with antennas and ICs. We also show a small antenna designs to improve on the form factor}
%     \item \textbf{Finally, we build algorithms to sense phase from RFID reader reliably to sense the force robustly}
%     \item \textbf{Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 5000 contact points, both over the air and over a pork belly setup for in-body sensing, as well as in moving multipath scenarios, and 2 case studies to motivate possible applications}
% \end{itemize}

% Force ubiquiti
\noindent Force is an ubiquitous phenomenon in our daily environment, with any two objects in contact exerting forces onto each other. Therefore, force sensors are a simple and unique way to quantify ubiquitous contact phenomenon, and bridge the gap between the digital world and the real environment, with clear use cases in AR/VR and ubiquitous computing\cite{}. Further, these force sensors can enable myriad of diverse applications, from warehouse scenarios, orthopedic implants to robotics.
For example, we could sense the weight (force) of the packages in a warehouse setting, and use the sensed force for integrity of the packages~\cite{sensor_checking_weights}, since an empty or improperly packed package would apply a lower gravitational force. Similarly, an orthopedic implant equipped with a force sensor could measure the contact forces between the knee joints as the patient recovers post-surgery to categorize the implant health (shown in Fig.xx) and how well the body accepts the knee implant~\cite{sensor_check_knee_implants_1,sensor_check_knee_implants_2}. Another application area is robotics, where these force sensors can be used to better control the robots, for example while gripping a sensitive objects the robotic manipulator needs to quantify the forces it is applying~\cite{gripper_force_needed_1_fruit,gripper_force_needed_2_robotic}, and in surgical robots which have to be careful while interacting with body tissues so that they don't damage the tissues by applying excessive forces~\cite{force_needed_1_surgical_robot}. 
% in field of surgical robots which navigate in tight in-vivo spaces where the robot can 

However, these applications pose numerous challenges on force sensors, and hence the applications are not mainstream today. 
For example, consider the usecase of sensing forces sustained by the knee-implant.
In this scenario, the force sensors need to be thin enough to fit within the narrow gaps between the bones in the knee joint.
Further it needs to fit snugly to the uneven bone shapes in the knee joint.
Since the implant is located inside the body (in-vivo), it is not possible to carry a wire till the sensor, and thus the sensor has to be read wirelessly via a remotely located reader outside the body.
To enable wireless operation, we can not assume an active radio near the sensor to transmit the sensor readings, since batteries pose a risk of contamination inside body, as well as requirement of battery would not allow for thin sticker-like sensors.
Hence, the most ideal force sensor has to be thin and sticker-like form factor to fit snugly inside the joint, and at the same time support wireless operation without requiring a battery.

Now, in order to design such wireless sensors which don't require batteries, a key theme is to use a `joint communication and sensing paradigm'.
In other words, the sensor has to create a powerful transduction mechanism, which converts force information directly onto the fluctuations in wireless signals travelling to and fro the remotely located reader.
Then the reader can measure these fluctuations and hence measure the applied forces on the sensor, in a way the sensor performs joint communication as well as sensing of the applied force.
Unlike the typical approaches where sensing is a localized phenomenon like voltage changes etc, which need to be sensed separately, and then get communicated via active radios, both operations requiring batteries, joint communication sensing paradigms scratch the requirement of batteries by directly creating fluctuations in wireless signals between the reader and the sensor.

In this paper, we present \name which for the first time demonstrates these wireless force sensitive stickers (Fig. \ref{fig:intro_fig}a,b), which can be stuck to everyday objects (Fig. \ref{fig:intro_fig}c), as well as flexibly confirm to orthopedic implants (Fig. \ref{fig:intro_fig}d) and robots (Fig. \ref{fig:intro_fig}e), in order to meet these various applications. 
Specifically, \name develops a novel force sensitive sensor, which are mm-scale as shown in Fig. xx, and are energy efficient.
, and develops a novel force transduction mechanism that directly alters the Radio Frequencies (RF) wireless signals as the sensor deforms under applied forces. 
Furthermore, \name uniquely interfaces these mm-scale force sensors to RFID stickers, which is not only flexible sticker, but also allows for wireless interrogation of sensor via a remotely located RFID reader.
% This integration allows \name's flexible, mm-scaled, energy efficient force sensor to use the popular battery-free RFID backscatter modulation to achieve wireless communication without requiring a battery.
% also achieves wireless communication in a battery-free manner. 
% performance as RFID tags, but can modulate the sensor signals for wireless reading.
\name finally develops robust signal processing algorithms atop of the COTS RFID reader, to allow for reliable reading of applied forces on the mm-scale sensor, in variety of environments, and even in presence of moving objects in the environment, to achieve the vision of ubiquitous force sensing. 
This method of creating force sensitive RFID stickers easily meets the motivated applications of knee implant force sensing and ubiquitous weight sensing in warehouses, as well as have the potential to enable many more applications.
% The key insight behind \name's flexible, mm-scaled, energy efficient force sensor design is that the sensor basically encodes force information directly onto the RFID modulated wireless signals reflecting off from the sensor, integrated with popular battery-free RFID backscatter modulation gives a can easily meet xyz applications...  Furthermore, \name stickers has potential to enable many more applications. 

The first challenge for creation of such force sensitive stickers is how does the mm-scale sensor create measurable changes in the wireless signals reflecting off from the sensor.
The mm-scale force sensor under applied force would further create sub-mm deformations in the sensor geometry, and this sub-mm deformation need to be sensed remotely at readers which are located meters away from the sensor, at least 1000 times more distance than the created deformation.
A recent work which attempts the similar force transduction, required a large sensor (80mm), to create this measurable channel change. 
More specifically the sensor length (size) is proportional to the changes in the channel, and hence design of mm-scale sensors which create measurable wireless signal fluctuations requires a new transduction mechanism not based on the length of sensor. 
% Therefore, it is make challenging to create a small sub-mm sized sensor, on which deformations caused by applied forces create substantial signal fluctuations to be read off by a remotely located reader robustly in presence of all the environmental clutter and noise.
\name solves this challenge by indentifying the changes in sensor thickness as an attractive alternate mechanism instead of length of the sensor.
Essentially, change in sensor thickness due to applied force creates capacitance changes. \name uses this capacitance change phenomenon to create a new transduction mechanism that translates the load capacitance into phase change at RFID frequencies, which essentially enables a measurable $>10^{o}$ phase change, even from the sub-mm deformations, when the sensor is miniaturized to mm-scale.

% This transduction mechanism is similar to how varactors create phase shifts in RF circuits.
% Essentially, \name designs a mm-scale force sensitive varactor sensor at 900 MHz, which gives measurable phase changes even when the sensor is miniaturized. 
We provide a mathematical understanding of this new transduction mechanism and show a simple framework which can be used to design such mm-scale capacitive force sensors which transduces force to RF signal phases.
Further, we perform multiphysics simulations in order to solve both maxwell's equations for force impedance calculations, as well as solid mechanics equations for force deformation in order to model the transduction phenomenon and confirm the sensor design, as well as the required RF interfacing, to guarantee a measurable wireless channel phase change for the joint communication sensing paradigm proposed by \name. Thus, \name creates a power joint communication-sensing paradigm for force sensors that can scale to mm-scale sensors, and would be energy efficient, and modulate the RF signals with a phase shift proportional to applied force.
 
% \name has three design components central to the creation of such force sensitive stickers, introduction of a new transduction mechanism which maps applied forces to wireless signal fluctuations, 
% designing a mm-scale sensor which harnesses the new transduction mechanism and
% interfacing the fabricated sensors to RFIDs for batteryless and wireless operation.


% This mechanism effectively communicates information by creating fluctuations in the wireless channel between the reader and the sensor.
% Previous work \cite{} has used a linear relationship between contact length effect created by force formation versus the wireless channel phase for transduction mechanism.
% Henceforth, the requirements from this transduction mechanism would be to create measurable changes in wireless channel.

% However, with a mm-scale sensor, the deformations caused by applied forces would be further sub-mm, which pose a challenge to create any measurable wireless channel changes.

% If this sensor is naively miniaturized to even $10mm$, the total phase change would get $1.5^{o}$ which is not enough to be measurable at the reader~\cite{}. 



Next, we design an interface for \name sensor to the backscatter technology like RFIDs, which can directly modulate the force-to-phase shift onto the wireless channel of RFID tags and enable battery-free operation. Furthermore, it would also enable \name to support multiple force sensors concurrently as well, with RFID providing unique identity. 
% Previous efforts have attempted RFID based sensor integration, cut a small piece of RFID antenna and installed a sensor, which inadvertently lead to reduced range of operation and the readings become unreliable~\cite{}. 
% in order to modulate the phase shifted signals from the sensor so that the remotely located reader can discern the sensor reflection from the other signals it receives. 
% A naive approach could be to cut a small piece of the RFID antenna and attach the sensor between the cut pieces. 
% In comparison, \name makes a key observation that the \name sensor is purely capacitive, and thus has purely reactive impedance. 
\name makes a key observation that the \name sensor is designed to be purely capacitive, and thus has purely reactive impedance. 
When a purely reactive impedance is interfaced in parallel to the RFIDs, we obtain a pure phase shifted signal with no reduction in the magnitude of reflected signal.
Since \name sensor only affects phase and not magnitude, it does not disturb the operation of RFID energy harvester and hence does not reduce the RFID reading range.
% To do so, we interface \name's sensor to COTS RFID stickers via two 20$\mu$m tungsten wire filaments, and show that this interfacing does not impact the RFID range.
% Thus, it creates robust RFID modulated and phase shifted reflections from the sensor.
This interfacing with RFIDs without losing any range allows for robust wireless sensing which does not compromise the reading range, or the sensor signal strength.
% In addition to COTS RFID stickers, we also show a possible interfacing method of the sensor by creating a PCB pad for the sensor, similar to how capacitors have standard size pads (0603, 0805 etc) for PCB based interfacing. 
In addition, \name also creates custom RFID tags on flexible PCB substrates, and we utilize a self-designed small 1cm$\times$1cm spiral PCB printed antenna to further miniaturize the form factor of the sensor.
We also show how we can interface the \name sensor with existing commercialized RFID stickers in a standalone manner without requiring a PCB.

% The third challenge is signal processing algorithms..phase variations: delta phase as a reliable metric go slow here RFID reading
% todo for tomorrow: design choice enables robust reading 
Finally, we design novel signal processing algorithms to read the phase changes from the sensor using COTS RFID readers, which would enable immediately usability of \name. \name develops the force measurement via phase readings reported by the RFID reader. FCC compliant RFID readers hop across the 900-930 MHz RFID band every 200ms, which creates phase discontinuities in the reported phase. However, since \name sensor conveys the force information via change of phases, by taking differential phases over time, we can get rid of the random hopping offsets introduced.
This elimination of random phase offsets allows for collating consistent information across the 50 different RFID channels, which in turn allows improved sensing performance because of channel averaging of phases, giving the capability to read phase changes accurate to 0.5-1 degree, which allows to sense forces with 0.2-0.4 N resolution across the 0-6N sensing range.

To summarize, we present first design for a mm-scale force sensor which can transduce force onto wireless signals at RF frequencies and integrate them with flexible RFIDs to attain the sticker form factor battery-less force sensors. We prototype the sensor based on the optimized design in COMSOL for the knee implant force sensing and ubiquitous weight application, using ecoflex material for the sensor fabrication. We integrate the sensor with popular RFID chipsets, along with multiple different flexible antenna design which can be powered and read wirelessly. The fabricated sensor by itself is 1000x lower volume form factor as compared to recent past work ~\cite{wiforce} on wireless force sensors and is the first work to showcase an end-to-end battery-less wireless operation. 
% We have tested the sensor for multiple application in indoors.  
We experimental show that our results obtained are consistent with the proposed transduction mechanism of capacitance to phase changes.  Our key results include: $<$0.5 N sensing accuracy, tested over $>$ 10000 contact forces applied on the sensor, both over the air and over a pork belly setup for in-body sensing. We also test the sensor with people moving around and show that our signal processing algorithm has robustness of phase sensing to the dynamic multi-path as well. Furthermore, our experimental prototype matches closely with FEM multiphysics simulations in COMSOL. We also present in simulations using our framework could be used to develop sensor for different ranges of force, by choosing appropriate polymer.

Using the above sensor design, we also conduct two experimental case studies with our sensor. 
% The first case study involves the sensors on robots and sensing the force applied on the robot by the environment and allowing it for safe operation of the robot without harming tissues. 
In our first case study, we demonstrate reading the forces applied by knee joints using toy-knee kit, and accurately measuring these force even in-body experiments. Finally, in our second case studies, we put different quantities of objects in a package and read weight from the force stickers attached to the bottom of the package, to identify if the packages are meeting the integrity on number of items in the package. We believe \name could be sensed many more quantities beyond just force, and could be generalized to using even everyday WiFi devices as readers.   


==> requirements/requirements.tex <==
% !TEX root = paper.tex

\section{Requirements}\label{sec:reqs}

